The Chromatic Lagrangian: Wavefunctions and Open Gromov-Witten Conjectures

Inside a symplectic leaf of the cluster Poisson variety of Borel-decorated $PGL_2$ local systems on a punctured surface is an isotropic subvariety we will call the chromatic Lagrangian. Local charts for the quantized cluster variety are quantum tori defined by cubic planar graphs, and can be put in standard form after some additional markings giving the notion of a framed seed. The mutation structure is encoded as a groupoid. The local description of the chromatic Lagrangian defines a wavefunction which, we conjecture, encodes open Gromov-Witten invariants of a Lagrangian threefold in threespace defined by the cubic graph and the other data of the framed seed. We also find a relationship we call framing duality: for a family of "canoe" graphs, wavefunctions for different framings encode DT invariants of symmetric quivers.

==> errata.tex <==

red X in Theorem 4.1?

puncture dual to corresponding f before eq 4.3.1

along the global relation below Remark 4.2

Eq. (4.2.5) $Phi_a$ on the wrong side

Under Eq. (4.2.5), K should be cal not bold

z1 to z2 in Lemma 7.1, LHS

==> introduction-old.tex <==

\section{Introduction}
\label{sec:intro}

This paper exploits cluster theory to compute wavefunctions for Lagrangian branes in
threespace
and to make explicit conjectures about their all-genus open Gromov-Witten invariants.  For certain branes, these numbers also relate to the cohomologies of twisted character varieties and Donaldson-Thomas invariants of quivers. 
Two structural tools in the schema are the behavior under mutation and the dependence of quantities on phases and framings.  

\begin{center}
\begin{tikzpicture}[scale=1.2]
\newcommand*{\boff}{10}; \newcommand*{\aoff}{35}; \newcommand*{\rad}{3};
\coordinate (a) at (-.15,-1.4);
\coordinate (b) at (4,-2);
\coordinate (c) at (6,0);
\coordinate (d) at (2,2);
\coordinate (e) at (-.2,1);
\coordinate (f) at (-.6,0);
\coordinate (g) at (1.5,0);
\coordinate (h) at (4,-.7);
\draw[very thick] (a) to[out=300,in=180] (b) to[out=180+180,in=270] (c) to[out=90,in=0] (d) to[out=180,in=50] (e) to[out=230, in=90] (f) to [out=270, in=120] (a);
%\draw[thick] (a) to[out=300,in=180] (b) to[out=180+180,in=270] (c) to[out=90,in=0] (d) to[out=180,in=50] (e) to[out=230,in=120] (a);
\draw[thick,blue] (c) to [out=210,in=0] (h) to[out=180,in=0] (g) to[out=180,in=0] (f);
%\draw[thick,blue] (c) to[out=210,in=320] (e);
\node at (5,1.9) {$\mathcal P$};
\node at (-1,-.2) { $\mathcal M$};
\node at (4.5,.7) {\small$\mathcal P_\Gamma$};
\node at (2.8,.9) {\small$\mathcal P_{\Gamma'}$};
\node at (1.2,1.2) {\small $\mathcal P_{\Gamma_{\mathrm{neck}}}$};
\node at (.5,-.2) {\tiny $W_{\Gamma_{\mathrm{neck}}}\!\equiv\! 0$};
\node at (4.5,-.4) {\small $\mathcal M_\Gamma$};
\draw[thick,red] (4-.5,-.5+.866) -- (4-.5,-.5-.866);
\draw[thick,red] (4-.866,-.5-.5) -- (4+.866,-.5-.5);
\node[red] at (3.9,.2) {\tiny phase};
\node[red] at (4.15,-1.15) {\tiny framing};
\draw[thick,dotted] (4,-.5) circle (1cm);
\draw[thick,dotted] (.6,0) circle (1cm);
\draw[thick,dotted] (2.3,-.3) circle (1cm);
\end{tikzpicture}
\end{center}

Let $\cP$ be the symplectic cluster variety of Borel-decorated, $PGL_2$ local systems on a punctured
surface $S$ with unipotent monodromy around the punctures.  There is a Lagrangian
subvariety $\cM\subset \cP$ of decorated
local systems with trivial monodromy at the punctures.
Cluster charts $\cP_\Gamma$ of $\cP$ are labeled by cubic graphs $\Gamma$ on $S$,
or dually ideal triangulations.  They are algebraic tori, and can be identified with
rank-one local systems on a Legendrian $S_\Gamma$ in the five-sphere,
i.e. $\cP_\Gamma \cong H^1(S_\Gamma;\bC^*).$
Then $\cM_\Gamma := \cM\cap \cP$ is a subspace of a torus,
the explicit description
of which will lead to enumerative predictions, but will also depend on
further choices known as a \emph{phase}, \emph{framing}. and \emph{cone}.

Central to the strategy for calculation
is to understand the effects
of a mutation $\Gamma \rightsquigarrow \Gamma'$,
which is dual to a flop of a triangulation, and to understand its interaction
with phases, framings and cones.
The whole story has a quantization, conjecturally related to higher-genus open
Gromov-Witten invariants.

\subsection{Open Gromov-Witten Conjectures}
\label{sec:intro-ogw}

The cubic planar graphs $\Gamma$ that label cluster charts also describe Legendrian
surfaces $S_\Gamma$, which form asymptotic boundary conditions for
categories of branes.  Non-exact Lagrangian fillings $L\subset \bC^3$
asymptotic to $S_\Gamma$ have open Gromov-Witten (``GW'') invariants which
we conjecture, following the pioneering work of Aganagic-Vafa \cite{AV},
are predicted by the geometry of the brane moduli space $\cM_\Gamma
\subset \cP_\Gamma$.

A phase and framing $A$ allow us to identify the universal cover of $\cP_\Gamma$
with $T^*H^1(L),$ and if we write the corresponding lift of $\cM_\Gamma$ as the graph of $dW_\Gamma$, then
after choosing a cone (which we suppress from the notation),
we can conjecture that $W_\Gamma$ is the open Gromov-Witten
generating function:
\begin{quote}
\underline{Conjecture}:  

\begin{quote}$W^{(A)}_\Gamma$ is the generating function
of disk invariants and obeys Ooguri-Vafa integrality.  (See Conjecture \ref{conj:disks}
for details.)
\end{quote}
\end{quote}
This conjecture appeared in \cite{TZ}.


The cluster variety $\cP$ has a quantization, each chart $\cP_\Gamma$
of which can be identified, through a splitting and cone, with a quantum torus, $\cD$:
$x_i y_i = q y_i x_i,$ where $q = e^\hbar.$  Then
$\cM_\Gamma$ quantizes is an ideal $\cI$, and the left $\cD$-module
$\cD/\cI\cD$ is cyclic for a vector $\Psi_\Gamma$, which we conjecture is the
generating function of all-genus open Gromov-Witten invariants.
\begin{quote}
\underline{Conjecture}:  \begin{quote}$\Psi^{(A)}_\Gamma$ is the generating function
of all-genus open Gromov-Witten invariants and obeys Ooguri-Vafa integrality.  (See Conjecture \ref{conj:ogw}
for details.)\end{quote}
\end{quote}
The two conjectures
are related:
$\Psi_\Gamma^{(A)} \sim e^{W^{(A)}_\Gamma/\hbar}$ as $\hbar \to 0.$

Since all ideal triangulations are related by flips, every cubic planar graph of genus $g$ (meaning it has $2g+2$ vertices) can be obtained from $\Gamma^{\rm neck}_g$ through a sequence
of mutations. 
%For instance, if we mutate along $g$ of the $g+1$ edges of $\Gamma^{\rm neck}_g$ that separate the inside of the necklace from the outside,
%then we obtain $\Gamma^{\rm canoe}_g$.
Our rubric therefore leads to conjectures for Lagrangian fillings of nearly all such
Legendrian surfaces.\footnote{We say ``nearly all,'' since certain mutations are not allowed ---
see Definition \ref{def:allowablemutation}.}



%
%\subsection{Example}
%
%If $\Gamma_{\mathrm{neck}}^1$ is the necklace graph with $1+1$ beads
%\begin{tikzpicture}[scale=.4]
%\draw[thick] (1,0) circle (.3cm);
%\draw[thick] (0,0) circle (.3cm);
%\draw[thick] (0,.3) to[out=90,in=90] (1,.3);
%\draw[thick] (0,-.3) to[out=270,in=270] (1,-.3);
%\end{tikzpicture},
%then in a particular phase and framing, we get a coordinatization
%$\cP_{\rm{neck}}^1 \cong \bC^*_x\times \bC^*_y$
%and $\cM_{\rm{neck}}^1$ is cut out by the equation $y=1.$
%Lifting to $\bC_u\times \bC_v$, where $u=\log(x)$ and $v=\log(y)$,
%we see $\cM_{\rm{neck}}^1 = \mathrm{Graph}(dW_{\Gamma_{\mathrm{neck}}^1}),$ with
%$W_{\Gamma_{\mathrm{neck}}^1} = 0$.  Quantization gives $yx = qxy$
%and the left ideal $y-1=0$ leads to the functional equation
%$\Psi_{\Gamma_{\rm{neck}}^1}(qx) = \Psi_{\Gamma_{\rm{neck}}^1}(x)$ and
%is solved by $\Psi_{\Gamma_{\rm{neck}}^1} \equiv 1.$
%
%Mutation along either strand of the necklace
%yields $\Gamma = K_4,$ the edge graph of a tetrahedron
%\begin{tikzpicture}[scale=.4]
%\draw[thick] (0,0) circle (1cm);
%\draw[thick] (0,0)--(0,-1);
%\draw[thick] (0,0)--(.866,.5);
%\draw[thick] (0,0)--(-.866,.5);
%\end{tikzpicture}.
%The rules of mutation give $\Psi_{\Gamma}=\Phi(x;q):=
%\prod_{n\geq 1}\frac{1}{1-q^nx}$, the quantum dilogarithm.
%We can see this directly, as follows.
%Now $S_{\Gamma} \cong T^2$ is a two-torus, and so $\cP_\Gamma \cong \bC^*\times \bC^*$
%after choosing a phase and framing.  In this case, the three phases defined by
%the Harvey-Lawson smoothings are all related to a given one $L$
%by permuting the coordinates in $\bC^3,$
%and the different framings of a given phase are determined by a single integer, $A$.
%The choice of phase and framing gives coordinates $x$ and $y$ in which
%the torus is $\bC^*_x \times \bC^*_y,$ and $\cM_\Gamma$ is cut out by the equation
%$x + x^Ay = 1.$  to lift $\cM_\Gamma$ to $T^*H^1(L;\bC)\cong T^*\bC_x\cong
%\bC_u \times \bC_v,$ where $u = \log(x)$ and $v = \log(y).$  Finding $W_\Gamma^A$ means
%solving $\partial_u W_\Gamma^A(e^u).$  For example, when $A = 0$ this says
%$\partial_u W_\Gamma = -\log(1-x),$ so $W_\Gamma = \Li_2(x)$.
%The quantized algebra of functions $\cD$ in these coordinates is $yx=qxy$, and when $A=0$ the
%left ideal $(x+y-1)\cD$ is cyclic for a function $\psi_\Gamma(x)$ obeying
%$\Psi_\Gamma(qx) = (1-x)\Psi_\Gamma(x)$.  This has a solution
%$\Psi_\Gamma(x) = \Phi(x;q),$ as we saw above.
%Then $W_\Gamma(x)$ is a semiclassical approximation:  $\Psi_\Gamma \sim \exp(W_\Gamma/\hbar)$ as $\hbar\to 0,$ where $q = e^\hbar,$
%a standard identity (see, e.g., \cite[Section II.D]{Z}).
%

\subsection{Analytic Aspects and Integrality}

One wants a description of the wavefunction in a cluster chart, whatever the
phase or framing --- and one wants integrality to hold.

The symplectic group acts transitively on the space of phases and framings.
It is generated by:  1) changes of basis of the phase subspace, or more precisely
their symplectic lifts; 2) changes of framing for a given phase; and 3) Fourier
transform, which interchanges phase and framing subspaces.
The problem with the previous treatment of the wavefunction in terms of
quantum dilogarithms is that the
quantum dilogarithm $\Phi(x;q)$ is an algebraic function without a well-defined
Fourier transform.

Instead, one wants to work its nonperturbative/analytic
analogue, the \emph{noncompact quantum dilogarithm}.\footnote{Physical
considerations as in \cite[Section 7]{CCV}
and \cite[Section 3]{CEHRV}
lead to this function more directly, where the noncompact quantum dilogarithm
arises as the partition function of a chiral multiplet in an effective three dimensional
$\cN=2$ supersymmetric theory on the sphere.
The noncompact quantum dilogarithm was identified in \cite{D} as being
appropriate for the present purpose.}
This is a meromorphic function $\varphi(u)$ on the complex plane, with
good convergence along certain rays to infinity, enabling a definition of its
Fourier transform.  The function $\varphi$ obeys many nice identities and functional relations akin to the gamma function --- see \cite{V} for an exposition.

Integrality in the analytic set-up
means that the analytic wavefunction $\psi_\Gamma$ has a product
expansion
$$\psi_\Gamma(u,\hbar) = \prod_{d\in \bZ_{\geq 0}^g\setminus \{0\}}\;\prod_{s\geq 0} \;\varphi(d\cdot u - \red{N} c_\hbar)^{n_{d,s}},$$
where
$u = (u_1,...,u_g),$
$c_\hbar = \frac{i}{2}(\hbar + \hbar^{-1}),$
 and $n_{d,s}\in \bZ$ are Ooguri-Vafa invariants.
Now one wants the symplectic group to act on $\psi_\Gamma$
to preserve the integrality of this product expansion --- in particular, Fourier transform.
Will this hold at all, and if so, will it hold for general integers $n_{d,s},$ or are
the Ooguri-Vafa invariants highly constrained by the requirement?

We don't know, and we cannot prove that integrality is preserved in general, but we have
checked several examples of our calculational schema and have found that
integrality holds because of several nontrivial Fourier-transform identities
of the noncompact quantum dilogarithm.

\subsection{Framing Duality}



Our starting point is the following observation about the
dependence on the phase/framing parameter $A = (h)$, a $1\times 1$ matrix,
when $\Gamma$ is the tetrahedron
graph and $S_\Gamma$ is the Legendrian Clifford torus:\footnote{
The twisted character variety of a genus-$h$ surface is the set of
isomorphism classes of irreducible representations of a central extension of the
fundamental group, i.e.~$n\times n$ matrices $A_1,...,A_h,B_1,...,B_h$ such that
$[A_1,B_1][A_2,B_2]\cdots [A_h,B_h] = \zeta,$ with $\zeta$ a central
$n$th root of unity, modulo
conjugation.}
\begin{equation}
\label{eq:modulo-HRV}
n^{(h)}_d = \dim H^{\mathrm{middle}}\left(\begin{array}{c}\text{``twisted'' character variety of rank $d$}\\
\text{local systems on a genus $h$ surface}
\end{array}\right).
\end{equation}
We are able to prove the equality assuming a conjecture of H\"ausel-Rodriguez Villegas \cite{HRV}.  Note that the $n^{(h)}_d$ are \emph{disk} invariants --- no higher genus surfaces were considered!
The relevant HRV conjecture relates the right-hand side of \eqref{eq:modulo-HRV} with the Donaldson-Thomas (``DT'') series of the quiver with one node and $h$ loops. 
Thus $(h)$
is the adjacency matrix, a perspective which generalizes nicely.

A special role is played by the Legendrian Clifford torus
and its higher-genus generalizations.
These Clifford surfaces of genus $g$ arise from ``canoe'' graphs (see
Figure \ref{fig:necklacecanoe}).
%When $\Gamma = \Gamma_{\rm{canoe}}^g$ is the ``canoe'' with $g$ seats
%$$
%\begin{tikzpicture}[decoration=brace]
%%\filldraw[fill=white!40!white, draw=black] (,0) circle (1cm);
%\draw[thick] (-4,-.5) ellipse (2cm and 1cm);
%\filldraw[fill=white!40!white, draw=black] (2-4,-.5) circle (.3cm);
%\filldraw[fill=white!40!white, draw=black] (-2-4,0-.5) circle (.3cm);
%\filldraw[fill=white!40!white, draw=black] (.8-4,.9-.5) circle (.3cm);
%\filldraw[fill=white!40!white, draw=black] (-.8-4,.9-.5) circle (.3cm);
%\filldraw[fill=white!40!white, draw=black] (1.51-4,.63-.5) circle (.3cm);
%\filldraw[fill=white!40!white, draw=black] (0-4,1-.5) circle (.3cm);
%\draw[decorate, yshift=2ex]  (-6,1) -- node[above=0.4ex] {$g+1$ beads}  (-2,1);
%\node[blue,thick] at (-4,-.6) {$\Gamma^{\rm neck}_g$};
%%\draw[very thick, dotted] (0,0) arc (135:150:2cm);
%\draw [black,very thick,dotted,domain=125:155] plot ({2.2*cos(\x)-4}, {1.2*sin(\x)-.5});
%\node at (0,0) {$\bullet$};
%\node at (1.2,.8) {$\bullet$};
%\node at (1-.2,-.8) {$\bullet$};
%\node at (2.2,.8) {$\bullet$};
%\node at (3.2,.8) {$\bullet$};
%\node at (4.2,.8) {$\bullet$};
%\node at (5.2,.8) {$\bullet$};
%\node at (6.2,.8) {$\bullet$};
%\node at (2-.2,-.8) {$\bullet$};
%\node at (3-.2,-.8) {$\bullet$};
%\node at (4-.2,-.8) {$\bullet$};
%\node at (5-.2,-.8) {$\bullet$};
%\node at (6-.2,-.8) {$\bullet$};
%\node at (7,0) {$\bullet$};
%\node at (3.7,.8) {$\cdots$};
%\node at (3.3,-.8) {$\cdots$};
%\draw (0,0)--(1.2,.8)--(2.2,.8)--(3.2,.8)--(3-.2,-.8)--(2-.2,-.8)--(1-.2,-.8)--(0,0);
%\draw (7,0)--(6.2,.8)--(5.2,.8)--(4.2,.8)--(4-.2,-.8)--(5-.2,-.8)--(6-.2,-.8)--(7,0);
%\draw (1.2,.8)--(1-.2,-.8);
%\draw (2.2,.8)--(2-.2,-.8);
%\draw (3.2,.8)--(3-.2,-.8);
%\draw (4.2,.8)--(4-.2,-.8);
%\draw (5.2,.8)--(5-.2,-.8);
%\draw (6.2,.8)--(6-.2,-.8);
%\draw (0,0) .. controls (-.8,-2.8) and (8,-2.8) .. (7,0);
%\node[blue,thick] at (3.5,-1.5) {$\Gamma_g$};
%%\draw [decoration={brace}, decorate] (1,1) -- (6,1);
%\draw[decorate, yshift=2ex]  (1.2,1) -- node[above=0.4ex] {$g$ seats}  (6.2,1);
%\end{tikzpicture}
%$$
\begin{figure}
\begin{tikzpicture}
\pgfmathsetmacro{\g}{5}
\pgfmathsetmacro{\gmin}{\g-1}
\pgfmathsetmacro{\gmid}{\g/2}
\pgfmathsetmacro{\gone}{\g/3+1/3}
\pgfmathsetmacro{\gtwo}{\g/3+\g/3+2/3}
\pgfmathsetmacro{\size}{.33}
\pgfmathsetmacro{\nodesize}{.06}
\pgfmathsetmacro{\min}{.7}
\node at (\gmid,-\min/2) {$\Gamma_{\rm{neck}}^g$};
\draw[fill] (\g-\size,.5) circle (\nodesize cm);
\draw[fill] (\g+\size,.5) circle (\nodesize cm);
\foreach \i in {0,...,\gmin}
{\draw[thick] (\i,.5) circle (\size cm);
\draw[fill] (\i-\size,.5) circle (\nodesize cm);
\draw[fill] (\i+\size,.5) circle (\nodesize cm);
\draw[thick] (\i+\size,.5) -- (\i+1-\size,.5);}
\draw[thick] (\g,.5) circle (\size cm);
\draw[thick] (0-\size,.5) to[out=180,in=180] 
(0-\size/2,-\min) to[out=0,in=180] (\gone,-\min)
to[out=0,in=180] (\gtwo,-\min) 
to[out=0,in=180] (\g+\size/2,-\min) to[out=0,in=0] (\g+\size,.5);
\end{tikzpicture}
\qquad
\begin{tikzpicture}
\pgfmathsetmacro{\g}{5}
\pgfmathsetmacro{\seatsize}{.8}
\pgfmathsetmacro{\gmin}{\g-1}
\pgfmathsetmacro{\gmid}{\g*\seatsize/2+.5}
\pgfmathsetmacro{\size}{.06}
\node at (\gmid,-.4) {$\Gamma_{\rm{canoe}}^g$};
\draw[fill] (0,\seatsize/2) circle (\size cm);
\draw[thick] (0,\seatsize/2) -- (1,0);
\draw[thick] (0,\seatsize/2) -- (1,\seatsize);
\draw[fill] (1+\gmin*\seatsize+1,\seatsize/2) circle (\size cm);
\draw[thick] (1+\gmin*\seatsize+1,\seatsize/2) -- (1+\gmin*\seatsize,0);
\draw[thick] (1+\gmin*\seatsize+1,\seatsize/2) -- (1+\gmin*\seatsize,\seatsize);
\draw[thick] (1+\gmin*\seatsize,0) -- (1+\gmin*\seatsize,\seatsize);
\draw[fill] (1+\gmin*\seatsize,0) circle (\size cm);
\draw[fill] (1+\gmin*\seatsize,\seatsize) circle (\size cm);
\foreach \i in {1,...,\gmin}
{
\pgfmathsetmacro{\ival}{1+\i*\seatsize-\seatsize}
\draw[thick] (\ival,0)--(\ival,\seatsize);
\draw[thick] (\ival,0)--(\ival+\seatsize,0);
\draw[thick] (\ival,\seatsize)--(\ival+\seatsize,\seatsize);
\draw[fill] (\ival,0) circle (\size cm);
\draw[fill] (\ival,\seatsize) circle (\size cm);
}
\draw[thick] (0,\seatsize/2) to[out=270,in=180] (\gmid,-.8) to[out=0,in=270] (1+\gmin*\seatsize+1,\seatsize/2);
\end{tikzpicture}
\caption{Mutating the necklace graph $\Gamma_{\rm{neck}}^g$ (left) along the
$g$ short strands results in the canoe graph $\Gamma_{\rm{canoe}}^g$ (right).
Here $g=5.$  The Legendrian surfaces generalize the Chekanov and Clifford tori,
respectively, which arise when $g=1.$}
\label{fig:necklacecanoe}
\end{figure}
The Clifford surfaces arise from mutations of the higher-genus version of the Chekanov torus, a genus-$g$ Legendrian surface corresponding to a ``necklace'' graph (see again Figure \ref{fig:necklacecanoe}).  Each Chekanov surface
has a distinguished exact Lagrangian filling and therefore 
a distinguished phase and no holomorphic disks:  $W_{\Gamma_{\rm{neck}^g}}\equiv 0$
and $\Psi_{\Gamma_{\rm{neck}^g}}\equiv 1.$
After mutation,
we get a distinguised phase for the Clifford surface $S_{\Gamma_{\rm{canoe}}^g}$,
i.e.~Lagrangian fillings $L$ with $\partial L = S_{\Gamma_{\rm{canoe}}^g}$
and $b_1(L)=g$, though
the different framings in this phase are parametrized by a $g\times g$ symmetric
integral matrix, $A$ (we often use the same letter to indicate a splitting),
and
\red{an identity allows us to
assume without loss of generality that $A$ has non-negative entries.}
The corresponding
wavefunction $\Psi^{(A)}_{\Gamma_{\rm{canoe}}^g}$
can be computed from cluster theory as in Section \ref{sec:intro-ogw},
and as we stated there
is conjecturally the partition function of the open topological string.

%
%More generally, for any genus $g$ there is a distinguished ``canoe'' graph $\Gamma^{\rm canoe}_g$ (a $g$-fold blow-up of the $\Theta$ graph --- see Figure \ref{fig:canoe})
%and a family of Lagrangians $L$
%with $b_1(L) = g$ which are asymptotic to a genus-$g$ hyperelliptic Legendrian.
%One chooses a phase and a framing, indexed by a symmetric $g\times g$ integer-valued matrix $A$. 
%An identity allows us to
%assume without loss of generality that $A$ has non-negative entries.

%Fixing such an $L\subset \bC^3$ and splitting $A$,
%the generating function of open Gromov-Witten invariants is called the superpotential $W_{\Gamma_{\rm canoe}^g}^{(A)}$, and appears as the semi-classical limit
%of the all-genus topological string partition function
%$\Psi^{(A)}_{\Gamma_{\rm{canoe}}^g}$. 
%Both of these depend on the framing $A,$ as indicated. 

 
We can now state our ``framing duality'' in the following way.
Let $Q_A$ be the symmetric quiver with $g$ nodes and adjacency matrix $A$.
Recall that the DT series is
the generating function for cohomologies of quiver representations
over different dimension vectors.  Then we have:
\begin{equation}
\label{eq:framingduality}
\text{$\Psi_{\Gamma_{\rm canoe}^g}^{(A)}$ is the DT series of $Q_A$}.
\end{equation}

\begin{remark}
Many of the results which establish this equality were
performed by Kontsevich-Soibelman in \cite{KS}.
For the genus-one case studied by Aganagic and Vafa, the connection between DT invariants and open GW invariants in different framings  was observed also in \cite{LZ}.  
As for other Legendrians, also in genus-one,
wavefunctions for knot and link conormals were considered in \cite{AENV}. 
We know
of no quiver dual for their framings \red{quiver-knot correspondence????}
For while the relationship \eqref{eq:framingduality}
suggests that the quiver invariants arise from an effective
quiver quantum-mechanical theory described by the capping data for
our noncompact threefolds made up from Harvey-Lawson
components (see, e.g. \cite[Section 5.1.1]{CEHRV}), we know of no direct physical argument
for the correspondence.  \red{quiver-knot correspondence}


\end{remark}


\begin{remark}
One wonders if the above relations extend to other cubic graphs and/or
nonsymmetric quivers.
\end{remark}

\subsection{Seminal Prior Works}

%For all other (non-canoe) graphs $\Gamma$ and their associated Lagrangians $L \subset \bC^3,$ we compute $\Psi^{(A)}_\Gamma$ by
%exploiting cluster theory:  we can relate graph mutations to cluster mutations.
%Specifically, we begin with the necklace graph $\Gamma^{\rm neck}_g$ with $g+1$ ``beads'' --- see Figure \ref{fig:necklace}.
%It is a higher-genus analogue of the Chekanov torus ($g=1$), and has an exact Lagrangian filling $L$ by a genus-$g$ handlebody.
%Since $L$ is exact, it is unobstructed and has superpotential $W = 0$ and wavefunction $\Psi = 1.$

Very similar constructions were considered from related physical perspectives
in prior works.
In \cite{CEHRV} and \cite{DGGo} the authors consider an M5-brane on $S^3\times L,$ where $L$ is a Lagrangian
submanifold of a compactifying space.  (Those authors call this Lagrangian $M$.)
They describe the partition function of the effective 3d theory on $S^3$ as a quantum-mechanical state. 
The M-theory set-up expresses this partition function as an integer combination of dilogarithms.
The partition function can also be computed by reduction to $L$.
It is a general property of quantum field theory that 
the path integral on a manifold with boundary always defines
a state in the Hilbert space defined by the boundary.
In the present case the boundary Hilbert space is the quantization of the space of flat $\mathrm{U}(1)$ connections on the genus-$g$ Legendrian boundary surface $S_\Gamma.$
The wavefunction $\psi$ should be understood as the wavefunction of this
quantum state. \red{(The solution is global, in that we have a quantization....)}






In fact, many of the results of this paper have appeared in various contexts in
important previous works, to which we owe a debt of gratitude.
Most notable are:  \cite{CCV} and particularly \cite{CEHRV}, which
are closest, and which studied the
behavior of these wavefunctions under symplectic transformations, though
not via cluster theory and did not relate the results to Gromov-Witten invariants;
\cite{DGGo} and \cite{DGGu}, which overlap with the present paper and \cite{CEHRV} in considering Lagrangian
double covers branched over tangles, and which
studied the corresponding Lagrangian moduli space;
\cite{KS}, which studied quiver representations
and preservation of integrality under changes of framings, providing
many of the key formulas that we use;
finally, some of the material here was discussed in \cite{TZ}, \cite{Za} and \cite{LZ}.
Further citations are made in the text.

\subsection*{Acknowledgements}

We are greatly endebted to David Treumann, who was involved in a large part of this collaboration.
\red{It is a pleasure to thank...} Roger Casals, Lenny Ng and Boris Tsygan for helpful conversations.
We thank Peng Zhou for asking about mutations very early in this project. 
We thank Jake Solomon and Sara Tukachinsky for discussing the role of framings in their work.
L.S.~ has been supported by NSF grant DMS-2200738.
E.Z.~has been supported by NSF grants DMS-1406024,
DMS-1708503 and DMS-2104087.



==> outline.tex <==

This is not a .tex file, but a place to hold a conversation which is more permanent than chat and easier to return to and edit than e-mail.  PLEASE EDIT AND CORRECT.  I am done with this draft for now.  -Eric


COMMENTS

Should [11] be folded into [4]? -Eric
Maybe [7] and [8] should be merged.

PRINCIPLES

* Be open about what is duplicated or translated from other math or physics papers.
* Be clear about what is new.




WHAT WE DO (reorder as you find appropriate)

*[1] Define quantized cluster variety of framed local systems on surfaces.  (Duplicated from Fock-Goncharov, Goncharov-Shen). % Linhui can write this part

*[2] Define quantum Lagrangian ideal, cyclic for a defining "wavefunction".  (Translated from Dimofte-Gabella-Goncharov) 

*[3] Identify classsical charts as local systems on Legendrian surfaces and Lagrangian subvariety as Fukaya/sheaf moduli space.  (Duplicated from Treumann-Z)

*[4] Definition of phase and framing.  (Treumann-Z)

*[5] Integrality of wavefunction and preservation under change of framing (duplicated from Kontsevich-Soibelman); behavior under mutation along "position" edges.

*[6] Conjectural equivalence of wavefunction with all-genus open Gromov-Witten invariants (part new, part Treumann-Z)

*[7] Framing duality:  Equivalence of wavefunction for canoe graph in framing A with DT series of symmetric quiver with adjacency matrix A.  (part new; math lifted from Kontsevich-Soibelman)

*[8] Relation to invariants of character varieties a la Hausel-Rodriguez-Villegas (new?)

*[9] The analytic story:  wavefunction for canoe via noncompact quantum dilogarithm and behavior under mutations and change of phase (part new [conventions.pdf], part in CEHRV Sec. 5 and CCV Sec. 8)

*[10] Integrality conjecture (as above with CEHRV and CCV)

*[11] Hamiltonians, phases and pants decompositions (new, in-progress)


SECTION HEADINGS

... pending discussion of the above, with tentative assignments

Title?

[1]:  Introduction  %%% Eric+

[2]:  Cluster varieties of framed local systems  %%% Linhui

[3]:  The Lagrangian ideal of trivial holonomies  %%% Linhui

[4]:  Cubic planar graphs and Fukaya moduli  %%% Eric

[5]:  Phases and framings  %%% (to incorporate [11]?) Eric

[6]   Integrality and Open Gromov-Witten conjectures  %%% (to incorporate [6] above?) Eric

[7]:  Framing Duality  %%% (to incorporate [8] above?)  Eric+

[8]:  The analytic picture   %%% Gus?

[9]:  Integrality for the analytic wavefunction

[A]:  Notation and conventions

==> phasesandframings.tex <==


\section{Phases and Framings}
\label{sec:phasesandframings}

Phases and framings will allow us to extract enumerative information from the moduli
space of framed local systems. 

\subsection{Definitions and Context}

\begin{definition}
\label{def:phaseandframing}
Let $H\cong \bZ^{2g}$ be a rank-$2g$ lattice with a non-degenerate, antisymmetric pairing $\omega.$ 
A \emph{phase} is a rank-$g$ isotropic subgroup $K\subset H$.  A \emph{framing} of $K$
is a transverse isotropic subspace.
We call the combination of phase and framing an \emph{isotropic splitting}, or sometimes
just \emph{splitting}.
\end{definition}

We will be studying phases and framings when $H = H_1(\Lambda)$ is the homology
of a genus-$g$ surface, $\Lambda$ and $\omega$ is the intersection pairing.
So let $L$ be an orientable three-manifold with boundary a genus-$g$ surface $\Lambda = \partial L$, with  $H_2(L)=0$. Then it follows from the long exact sequence in homology together with the Poincar\'e-Lefschetz duality isomorphisms $H^1(L)\simeq H_2(L,\Lambda), H_1(L,\Lambda)\simeq H^2(L)$ that $b_1(L)=g,$\footnote{In this section,
homology will be taken with $\bZ$ coefficients unless otherwise stated.}
so that we obtain the short exact sequence
%$$
%0\rightarrow H^1(L)\to H_1(\Lambda) \to H_1(L)
%\to 0.
%$$
%By \cite[Lemma 3.5]{H}, the map $\pi: H_2(L,\Lambda) \to H_1(\Lambda)$ has rank
%$g = \frac{1}{2}b_1(\Lambda).$  
%Since the rank of $H_1(\Lambda)=2g,$ the image of $H_1(\Lambda)\to H_1(L)$
%has rank $g$ and therefore $\pi$ is surjective.
%We therefore have a short exact sequence, which by
%Poincar\'e-Lefschetz duality isomorphism $H^1(L)\cong H_2(L,\Lambda)$
%we can write as
%\begin{equation}
%\label{eq:ses} 0\to H^1(L)\to H_1(\Lambda)\to H_1(L)\to 0.\end{equation}
\begin{equation}
\label{eq:ses}
\xymatrix{0 \ar[r]& H^1(L) \ar[r]& H_1(\Lambda) \ar[r]^{\pi} & H_1(L) \ar[r] & 0} 
\end{equation}

The notion of phases and framings will apply to above geometic setting.

\begin{definition}
\label{def:geometricphase}
Suppose $H = H_1(\Lambda)$ is the first homology of a genus-$g$ oriented surface $\Lambda$,
and $L$ is an orientable three-fold with $\partial L = \Lambda$. 
We have the short exact sequence of Equation \ref{eq:ses}.
We say that a phase $K\subset H$ is \emph{geometric} if $K = Ker(\pi)\cong H^1(L).$
An accompanying framing is an $\omega$-isotropic splitting
$\iota: H_1(L)\hookrightarrow H_1(\Lambda)$ of the short exact sequence \eqref{eq:ses}.
\end{definition}


In the context of open Gromov-Witten theory, $\Lambda$ is
Legendrian in a contact manifold and $L$
is Lagrangian in a symplectic filling.
%
%Let $L$ be a Lagrangian filling of a genus-$g$ Legendrian surface $\Lambda = \partial L$ with $b_1(L)=g.$
%Let $\omega$ be the nondegenerate, antisymmetric intersection pairing on $H_1(\Lambda).$ 
%A \emph{phase} is
%an $\omega$-isotropic rank-$g$ sublattice $K \subset H_1(\Lambda)$.  A
%\emph{framing} of $K$ is a rank-$g$ $\omega$-isotropic subspace transverse to $K.$
%\end{definition}
%
%\red{Should we try to define this independent of the geometric context of a filling?
%Do we want to make the phase the kernel of $\pi$ or dissociate the two?}
%
%In other words, ${\mathrm Ker}(\pi)$ is a phase
%and a framing is a splitting of the sequence in Equation \ref{eq:ses},
%a transverse lattice which we can identify with $H^1(L)$.
%

\begin{remark} In \cite{TZ}, the above geometric phases
were called ``OGW framings" to
connote open Gromov-Witten theory.  The definition was generalized from \cite{AKV},
where mirror symmetry was used to make
conjectures in open Gromov-Witten theory.\footnote{In \cite{I} a similar definition of framing is made, but without the isotropic condition.}  The terminology
stems from the connection to Chern-Simons theory through large-N duality,
where Lagrangians are knot conormals and framing relates to the framing of knots.
We describe the connection to open Gromov-Witten theory later in this section.  
\end{remark}


\begin{remark}
Here is why we need phases and framings.
Let $\cX = \cX_{PGL_2,S^2}$ be the cluster variety of framed local systems on a sphere.  Let $\cP$ be the symplectic leaf of unipotents, and let $\cM$ be the Lagrangian subvariety defined by trivial monodromy.\footnote{\red{Twisted local systems?}} Let $\Gamma$ be a cubic graph on the sphere $S = S^2$ and $S_\Gamma \subset J^1(S)$ the associated a Legendrian surface up to isotopy.  We write $\cP_\Gamma = H^1(S_\Gamma;\bC^*)$ for the corresponding cluster chart.
A splitting allows us to write $H^1(S_\Gamma;\bC^*)$ as
$T^*(H^1(L;\bC^*))/H_1(L)$.
When we lift $\cM$ to $T^*H^1(L;\bC^*)$ we can write it locally as the
graph of the differential of a function $W_\Gamma$ on $H^1(L;\bC^*)$, from which we will
extract enumerative information.
\end{remark}


Recall from \cite{TZ} the combinatorial model of the first homology of a Legendrian
$\Lambda:=S_\Gamma$
defined from a cubic planar graph $\Gamma$ on a sphere, $S$:
we have
$H_1(S_\Gamma) \cong \bZ^{E_\Gamma}/\!\sim$, given by the lattice of edges modulo relations generated by faces:  $\sum_{e\in \partial f}e \sim 0.$  We have an antisymmetric pairing $\overline{\omega}$ on $\bZ^{\E_\Gamma}$,
depending only on the orientation of $S$, defined by $\overline{\omega}(e,e') = \pm 1$ if $e$ and $e'$ are adjacent to a vertex $v$ with $e$ preceding/following $e'$ in the cyclic ordering at the vertex
\begin{tikzpicture}[scale=.2]
\draw (-1.4,1)--(0,0)--(1.4,1);
\draw (0,0)--(0,-1.5);
\node at (-2.2,1) {$e'$};
\node at (.9,-.5) {$v$};
\draw[fill] (0,0) circle (.3cm) ;
\node at (2.2,1) {$e$};
\end{tikzpicture}, and zero otherwise.  
Since $\sum_{e\in \partial f}e$ generates the kernel of this pairing,
$\overline{\omega}$ descends to a nondegenerate, antisymmetric intersection pairing $\omega$
on 
\begin{equation}
\label{eq:h1}
H_1(S_\Gamma) \cong \bZ^{E_\Gamma}/\!\sim.
\end{equation}


\subsection{Foams}
\label{sec:foams}

A cubic graph $\Gamma$ on the sphere $S$ is dual to a triangulation of $S$.  If $\Gamma$ is three-connected, then by Steinitz's theorem it is the edge graph of a polyhedron.  A \emph{foam} $\bF$ is the dual structure to a tetrahedronization of the polyhedron:  it is a polyhedral decompsition of the three-ball $B$ with $\partial B = S.$ The data of $\bF$ includes the quadruple $(R,F,E,V)$ of regions, faces, edges and vertices.  The foam is \emph{ideal} if it is dual to an ideal tetrahedronization of $B$, meaning it has no internal vertices. Even if $\Gamma$ is not dual to a polyhedron, the notion of foam makes sense --- see \cite[Definition 3.1]{TZ}.

\subsubsection{The Harvey-Lawson Foam}
\label{subsec:hlfoam}

The foam $\bF_{\mathrm{HL}}$ of the Harvey-Lawson Lagrangian $L_0\subset \bC^3$
has a single vertex at the origin in $\bR^3,$
four edges $E_i$ equal to the rays $\bR_{\geq 0}\cdot v_i$
where $v_0 = (1,1,1)$ and $v_i = -v_0 + 2e_i$, with $e_i$ the standard basis vectors.
There are $6 = \binom{4}{2}$ faces $F_{ij}$
equal to the cones spanned by unordered pairs of edges,
and $4 = \binom{4}{3}$ regions equal to the cones spanned by triples of edges. 
(It can be succinctly described as the toric fan of ${\bf P}^3.$)




The singular, exact Harvey-Lawson Lagrangian $L_0$ in
$(\bC^3,\omega_{\mathrm{std}}=d\theta_{\mathrm{std}})$
is a branched $2:1$ cover of $\bR^3,$ branched over the over edges.
$L_0$ is a cone over $S^1\times S^1$ with parametrization
$(r,s,t) \mapsto (re^{is},re^{it},re^{-i(s+t)}) \in \bC^3$,
where $r\in \bR_{{\geq 0}}$ and $(s,t)\in S^1\times S^1.$
The covering map is the restriction to $L_0$ of $\bC^3\to \bR^3$
sending a complex triple to its real part:
explicitly $(r,s,t) \mapsto (r\cos(s),r\cos(t),r\cos(s+t)) \in \bC^3.$
The map is $1:1$ over the four rays with $(s,t) = (0,0), (\pi,0), (0,\pi),(\pi,\pi),$
which we think of as a singular tangle.
The six sheets of the foam are defined by $s = 0, s = \pi, t = 0, t = \pi, s+t = 0, s+t = \pi.$

The primitive function $f$ obeying $df = \theta_{\mathrm{std}}\vert_L$ is
$f = \frac{1}{4}r^2\left(\sin(2s)+\sin(2t)-\sin(2s+2t)\right).$  Note that $f$ is
odd under the hyperelliptic-type involution $(s,t)\leftrightarrow (-s,-t)$ and
$f=0$ along the preimages of the sheets of the foam.  Thus $f$ allows us to label the
branches of $L_0$ on the regions $R$.


\begin{center}
\begin{figure}[ht]
\includegraphics[scale=.14]{singular-foam.png}\hskip-.9in
\includegraphics[scale=.15]{deformed-foam.png}
\caption{One the left is the foam of the Harvey-Lawson Lagrangian:  there are $4$ rays bounding $6 = \binom{4}{2}$ sheets, which all meet at a point.  On the right is the deformed
foam of its smoothing.  Two sheets (pink) are smoothed to have hyperbolas as boundaries, while the boundaries of the other four consist of two halves of different hyperbolas, as well as the arc (green).}
\end{figure}
\end{center}

\subsubsection{Foams and singular exact Lagrangians}

From a foam $\bF$ we can define a singular exact (not necessarily special) Lagrangian $L_0$ locally modeled on the Harvey-Lawson cone and foam --- see \cite[Section 3.2]{TZ}.  As with the Harvey-Lawson cone
and foam, we can define a multi-valued function $f$ whose sign labels the branches of $L_0$
in the regions of the foam.  


\subsubsection{Deformation of the Harvey-Lawson foam}
\label{sec:hlfoamdef}

There are three distinct families of smoothings of $L_0$ corresponding
to the three matchings of the four
edges. 
We will describe the one for the matching $0\leftrightarrow 1, 2\leftrightarrow 3$;
the others are similar and are related by a permutation of
coordinates.
The smoothing $L_\epsilon$
has the topology of $\bR^2 \times S^1$ and has a parametrization in polar
coordinates 
$(r,s,t) \mapsto (\sqrt{r^2+\epsilon^2}e^{is},re^{it},re^{-is-it}) \in \bC^3$, which maps to 
$(\sqrt{r^2+\epsilon^2}\cos(s),r\cos(t),r\cos(s+t))\in \bR^3.$  
These are all diffeomorphic for $\epsilon \neq 0,$ and as we will be interested in topological
questions here we restrict to $L_1$ without loss of generality.
The branched cover is $1:1$ over the points with
$(s,t) = (0,0), (\pi,0), (0,\pi),(\pi,\pi),$ and these parametrize four rays $E_i$ which
trace out \emph{two} hyperbola components ($E_0\cup E_1 = \{x^2-y^2 = 1, y=z, x> 0\}$
and $E_2\cup E_3 = \{x^2-y^2 = 1, y=-z,
x < 0\}$), a smoothing of the singular
tangle of $L_0$. )

There is also the line segment $a \subset \bR^3$
between $(-1,0,0)$ and $(1,0,0)$ which we call an \emph{arc} --- it
is the image of $r=0.$  Note that $L_1\to \bR^3$ is $2:1$ over the arc.
The six sheets $F_{ij}$ now bound either a smooth edge $E_i\cup E_j$ if $(ij) = (01)$ or $(23)$,
or otherwise the union $E_i \cup E_j \cup a$.  This will be our local model of a deformed foam.
More generally,
let $s_i$ be the matching of edges of ${\bf F}_{\mathrm{HL}}$
which pairs $v_0$ and $v_i$.  We write ${\bf F}_{\mathrm{HL},s_i}$ for the local deformed foam.
Its arc is the line segment between $-e_i$ and $e_i$.

Away from the origin and the preimage of the arc, the Harvey-Lawson cone and its smoothing are homeomorphic:  $L_0\vert_{r\neq 0}\cong L_1\vert_{r\neq 0}$.  As a result, the same primitive function $f$ can be used to label regions of the foam and of its deformation, at least away from the
arc.  The local geometry of $L$ and the deformed foam near an arc is shown in Figure
\ref{fig:foam-upclose}.

\begin{center}
\begin{figure}[ht]
\begin{tikzpicture}
 \pgfmathsetmacro{\a}{5}
 \pgfmathsetmacro{\b}{-3}
  \pgfmathsetmacro{\c}{.707}
  \pgfmathsetmacro{\d}{.4}
    \pgfmathsetmacro{\s}{.3}
    \pgfmathsetmacro{\lift}{1.2}
    \pgfmathsetmacro{\n}{4}
    \pgfmathsetmacro{\nn}{2*\n}
    \pgfmathsetmacro{\ninv}{\n^(-1)}

\draw[fill,gray,opacity=.5] (-\a+\c*\d,\b-\d)--(\a+\c*\d,\b+\d)--(\a-\c*\d,\b-\d)--(-\a-\c*\d,\b+\d);
\draw[fill,gray,opacity=.5] (-\a+\c*\d,\b-\d)--(\a-\c*\d,\b-\d)--(\a+\c*\d,\b+\d)--(-\a-\c*\d,\b+\d);
\draw[green,very thick] (-\a,\b)--(\a,\b);
\draw[green,very thick] (0,0) ellipse (5 and 1);
\draw[fill,red] (\a,0) circle (.1);
\draw[fill,red] (-\a,0) circle (.1);
\draw[fill,red] (\a,\b) circle (.1);
\draw[fill,red] (-\a,\b) circle (.1);
\foreach \ii in {0,...,1}
{
\pgfmathsetmacro{\jump}{3.6*\ii}
\foreach \i in {0,...,\nn}
{
\pgfmathsetmacro{\k}{(\i - \n)*\ninv}
\pgfmathsetmacro{\kk}{\k*\k}
\pgfmathsetmacro{\testy}{0}
%{\pgfmathsetmacro{\j}{(\i - \n)}
\pgfmathsetmacro{\j}{\a*\k}
\draw[fill,green] (\j,\b+\lift+\jump) circle (.05cm) ;
\draw[thick,black] (\j - \s*1 ,\b+\lift+\jump - \s*\k)--(\j  + \s*1,\b+\lift + \jump + \s*\k);  
\draw[thick,black] (\j - \s*\k ,\b+\lift+\jump - \s*1)--(\j  + \s*\k,\b+\lift + \jump + \s*1);  
%\draw[fill,violet] (\j -.17,\b + \lift + \jump + .17) circle (.05cm);
\pgfmathsetmacro{\z}{(2*\ii-1)*(.17)*(1-\kk)^(1/2)}
%\node at (\j,0) {\kk};
\draw[fill,violet] (\j ,\b + \lift + \jump - \z) circle (.05cm);
}}
\foreach \i in {0,...,\nn}
{\pgfmathsetmacro{\k}{(\i - \n)/\n}
\pgfmathsetmacro{\j}{\a*\k}
\pgfmathsetmacro{\jump}{3.6}
\node at (\j + .35,\b + \lift + \jump + .35) {$+$};
\node at (\j - .35,\b + \lift + \jump - .35) {$+$};
}
\foreach \i in {0,...,\nn}
{
\pgfmathsetmacro{\k}{(\i - \n)/\n}
%\pgfmathsetmacro{\j}{(\i - \n)}
\pgfmathsetmacro{\j}{\a*\k}
\pgfmathsetmacro{\jump}{0}
\node at (\j + .35,\b + \lift + \jump + .35) {$-$};
\node at (\j - .35,\b + \lift + \jump - .35) {$-$};
}

\end{tikzpicture}
\caption{The neighborhood of an arc (the green line segment) and its lift to the Lagrangian (green oval).  Four sheets, forming two surfaces (gray) meet at the arc.  The cross-sectional planes are shown, along with the sign of the primitive function $f$ on $L$.  The red dots are where the sheets
$s = 0,\pi$ meet the arc, so the sign of $f$ changes as they are crossed.  The purple dot
is the cross section of the oriented loop $\gamma_a$ --- see Definition \ref{def:ordloop}.}
\label{fig:foam-upclose}
\end{figure}
\end{center}


\subsubsection{Deformed Foams}

\begin{definition}
Let ${\bf F}$ be a foam with vertex set $V$ consisting of $n:= \#V$ vertices.
Write $\cS$ for the set of matchings of half edges at each vertex, so $\#\cS = 3^n.$
Let $s\in \cS$.  We define a \emph{deformed foam} ${\bf F}_s$ to be any set of vertices,
edges, arcs, faces and regions which agrees with ${\bF}$ outside some $\epsilon$-neighborhood
of $V$ and which is homeomorphic to the local deformed foam
of ${\bf F}_{\mathrm{HL},s}$ of Section \ref{sec:hlfoamdef} within an $\epsilon$-ball
of each vertex.
\end{definition}


The smoothed Lagrangian $L$ is branched over a tangle $T\subset B,$ i.e.~$T$ is a one-manifold. 
The construction of $L$ from a deformed foam identities a particular
set of branch cuts we call \emph{arcs}.

\begin{definition}
Let $s_i$ be the smoothing of the Harvey-Lawson foam
which matches the ray $\bR_{\geq 0}\cdot v_0$
with $\bR_{\geq 0}\cdot v_i$, where $v_0$ and $v_i$ are as in Section \ref{subsec:hlfoam}. 
The \emph{arc} of the deformed Harvey-Lawson foam $\bF_{\mathrm{HL},s_i}$
is the line segment from
$-e_i$ to $e_i$.
An \emph{arc} of a deformed foam $\bF'$ is the locus in $B$ corresponding to the
arc of the Harvey-Lawson foam under the local identification of $\bF'$ with
$\bF_{\mathrm{HL},s_i}$.
We write $A$ for the set of arcs of a deformed foam $\bF'$.
\end{definition}

Given an arc $a$ of a deformed foam $\bF'$ and its associated branched double cover $\pi: L\to B,$
define $\lambda_a = \pi^{-1}(a).$  Since $\pi$ is $2:1$ over the interior of the arc and $1:1$ at its edges, $\lambda_a$ is a circle.  Note that $\lambda_a$ does not (yet) have a distinguished orientation.

\begin{center}
\begin{tikzpicture}
 \pgfmathsetmacro{\a}{2}
 \pgfmathsetmacro{\b}{-1.7}
\draw[green,very thick] (-\a,\b)--(\a,\b);
\draw[green,very thick] (0,0) ellipse (2 and .5);
\draw[fill,red] (\a,0) circle (.1);
\draw[fill,red] (-\a,0) circle (.1);
\draw[fill,red] (\a,\b) circle (.1);
\draw[fill,red] (-\a,\b) circle (.1);
\draw[thick,-stealth] (0,-.8)--(0,-1.4);
\node at (.3,-1.1) {$\pi$};
\node at (.5,-1.9) {$a$};
\node at (1,-.7) {$\lambda_a$};
\end{tikzpicture}
\end{center}


\begin{proposition}
\label{prop:lifts}
Let $T\subset B$ be a smooth tangle with no circle components arising from a smoothing
of an ideal foam $F$, and let $L\to B$
be the corresponding branched double cover with branch locus $T$. 
Then $$H_1(L)\cong H_1(B,T)$$ and is generated by the branch cuts
from the smoothing at each vertex of $F.$
\end{proposition}
\begin{proof}
\red{XXX.  I think the lemma as stated is wrong --- must include orientations better.
I think it still can be stated that arc lifts, in whatever orientation, generate $H_1(L).$}
Let $L$ arise as a smoothing of an ideal foam, $F$, with $n$ internal vertices.
Write $\pi: L\to B$ for the double cover map.  Note
that a path in $B$ ending in $T$ lifts to a loop $\widetilde{\gamma}$.
As we 
and a chain homotopy of paths lifts to a chain homotopy of loops.
We thus get a map $H_1(B,T)\to H_1(L).$  \red{NO -- orientations.}
Let $s_i$ be the $n$ short arcs between strands of the smoothing and call $t_i$ the corresponding
elements of $H_1(L)$.  We claim that these branch cuts $t_i$ generate $H_1(L)$ and therefore
the map $H_1(B,T)\to H_1(L)$ is an isomorphism.  This will prove the lemma.
(We may have $n>g,$ so there may be relations among the $t_i$.)

Define $L'$ by attaching $n$ disks $D_i$ such that the boundary of $D_i$ is identified with $t_i.$
We have the exact sequence 
\begin{equation}
\label{eq:LL'exseq}
H_2(L',L) \longrightarrow H_1(L) \stackrel{\pi}{\longrightarrow} H_1(L').
\end{equation}

Let $L''$ be the singular Harvey-Lawson cover of $B$ defined by $F$.  Note
that $L'$ and $L''$ are homotopy equivalent by a contracting homotopy which shrinks
$D_i$ to the $i$th vertex.  Therefore $H_*(L')=H_*(L'').$

By excision, we have
$H_2(L',L) \cong H_2(\sqcup D_i, \sqcup t_i) \cong \bZ^n,$ where the image in $H_1(L)$ of the
generators in $H_2(L,L')$ are the cycles $t_i$.

Since $B$ retracts to $F$, $L''$ retracts to $\pi^{-1}F$ which is homeomorphic to two copies of $F$ glued along $F_1$.  Call this space $D(F)$.  Similarly, call $D(B)$ the space constructed
as two copies of $B$ glued along $F_1.$  So $L''$ and $D(B)$ are homotopy equivalent.
Now $B$ is contractible, so for $i>0$, we have
$$H_i(L'') \cong H_i(D(B)) \cong H_i(D(B),B) \cong H_i(B,F_1)$$
\red{where the last identify is by excision.}
Now $H_i(B,F_1)\cong H_i(F,F_1) = 0$, so $H_1(L'')=H_1(L')=0.$
Therefore, by Equation \ref{eq:LL'exseq}, $\pi: H_2(L,L')\twoheadrightarrow H_1(L)$
is  surjection, the $t_i$ generate $H_1(L),$ and $H_1(L)\cong H_1(B,T).$

Finally, note that $H_1(B,T)$ has rank $g$, meaning the surjection $\pi$ is an isomorphism.
\end{proof}



\subsection{Tangles and Lagrangians}

We continue our study of Lagrangians arising from smoothings of foams.

Let $\Gamma \subset S$ be a cubic graph on the sphere, let $\bF$ be an ideal foam on the three-ball $B$, whose regions, faces and edges respectively bound the faces, edges and vertices of $\Gamma$.
Let $\cS$ be the discrete set of smoothings of $\bF$, i.e.~the set of matchings of edges incident to each vertex of $\bF$ --- so $\#\cS = 3^{\#V}.$  Let $s$ be a smoothing whose resulting tangle $T$
has no circle components.  Let $L$ be a smooth Lagrangian corresponding to the
deformed foam $\bF_s$.


Recall that for an arc $a$ we werite $\lambda_a := \pi^{-1}(a).$  We now define
an orientation on $\lambda_a$, thus definining an element $\gamma_a\in H_1(L).$

Since the construction of the smoothing is local, we need only look at the Harvey-Lawson
smoothing $L_1$ and its unique arc $a$, which we can lift to the \emph{parametrized}
curve $(e^{it},0,0)$ and take the induced orientation.  This is the
orientation induced from the unique holomorphic disk in $\bC^3$ bounding $L$,
i.e.~$|z_1|\geq 1.$  We can also
give a more combinatorial construction that does not require an explicit local
model, as follows.


\begin{definition}
\label{def:ordloop}
\red{
We choose a canonical orientation for $\lambda_a$ by
orienting the arc arbitrarily and taking
a push-off of the path along the arc that has some combinatorial properties, using
the primitive function, $f$.  We require that near the start of the arc, in the chosen
orientation, that $f$ has a negative value on the push-off and lies in one of
the two fat regions (see Figure \ref{fig:foam-upclose}),
i.e.~outside of two sheets which meet at the arc's origin,
then crosses once at the midpoint of the arc in a counterclockwise direction
(in the induced orientation of the transverse plane) and
then again crosses the origin of the transverse plane at the arc's endpoints. 
There two such push-offs, but the
resulting paths are homotopic. 
Likewise, the opposite orientation of the arc leads to a homotopic path.  For an arc $a$, write $\gamma_a$ the resulting element of $H_1(L).$}
\end{definition}

\begin{proposition}
The prescription in Definition \ref{def:ordloop} is similar to how
unoriented edges of a cubic planar graph
lead to an oriented loop of the associated branched cover --- see \cite[Section 4.6]{TZ} ---
albeit somewhat more intricate.
\end{proposition}

\begin{proposition}
Let $L$ arise as a smoothing of a foam $\bF$ so that the associated tangle has no
circle components.  Write $A$ for the set of arcs of the deformed foam $\bF'$.
Then there is a canonical surjective map $\gamma: \bZ^A \twoheadrightarrow H_1(L)$
\end{proposition}
\begin{proof}
We know from Proposition \ref{prop:lifts} and Definition \ref{def:ordloop} that the arc lifts $\gamma_a,$ for $a\in A,$ 
generate $H_1(L)$.  
Therefore, the assigment $a\mapsto \gamma_a$ defines the desired surjective map $\gamma.$
\end{proof}


For each internal face, we will find a relation among the arc loops $\gamma_a$.
Together these relations characterize $H_1(L)$ as $\bZ^A/\sim.$
We begin with a combinatorial lemma.

\begin{lemma}
\label{lem:nminusr}
Let $\bF'$ be a deformed ideal foam with $n$ arcs and $r$ internal faces
so that the associated tangle $T \subset B$ has no circle components.
Suppose
$\partial \bF' = \Gamma \subset S$ is a cubic planar graph and $S_\Gamma$ has genus $g$.
Then $b_1(L) = g$, and we further have
$$g = n - r.$$
\end{lemma}
\begin{proof}
Suppose the undeformed foam $\bF$ has $n$ internal vertices (so $\bF'$ has $n$ arcs),
$r$ internal faces, and $i$ internal edges.  There are also $g+3$ boundary faces, $3g+3$ boundary edges, and $2g+2$ boundary vertices.
Note there are no internal regions by the ideal assumption, so the regions of $\bF$
are in correspondence with the $g+3$ faces of $\Gamma$.  Similar correspondences arise for faces and edges of the foam which meet the boundary.
Since $\chi(B) = 1,$ we have
$$1=[n +2g+2] - [(2g+2+3g+3+i)] + [(3g+3+r) +(g+3)] - [g+3],$$
or $1 = n - i + r$.  So $i = n + r - 1.$
Now the components of the deformed foam $\bF'$ differ in that each vertex of $\bF$ spawns two vertices of $\bF'$ as well as one arc, which lifts two line segmaents of $L$.  The  lifts under $\pi$ of
the components of the $\bF'$ (one for edges and boundary vertices, two for others) give a decomposition of $L$, and since $\chi(L) = 1 - g,$ we have
$$1-g = [2n + 2g+2]  - [2n + 2g + 2 + 2(3g + 3) + i] + [2(3g+3) + 2r + 2(g+3)] - [2(g+3)]$$
or
$1 - g = - i + 2r.$  Since $i = n+r-1$ from above, we have $1-g = 1 - n - r + 2r,$ so
$$g = n - r.$$
\red{XXX.  Use only internal faces from the start?}
\end{proof}

To define the relation, we need a careful discussion of the sign of an arc relative to a face. 

\begin{definition}
\label{def:arc-sign}
Let $F$ be a face of a deformed foam $\bF'$ bounding an arc $a\in A$.
Then we have a homeomorphism of a
neighborhood of $a$ with a neighborhood of the lone arc of the Harvey-Lawson deformed foam
$\bF_{\mathrm{HL},s_i}$
defined by some smoothing $s_i$ which pairs the edges containing vectors $v_0$ and $v_i$ ---
see Section \ref{sec:hlfoamdef}.  Let $F_{ij}'$ be the face of $\bF_{\mathrm{HL},s_i}$
corresponding to $F$,
which deforms the face $F_{ij}$ of $\bF_{\mathrm{HL}}$ containing $v_i$ and $v_j$ (note $i,j \in \{0,1,2,3\}$).
Let us orient the arc from the end bounding the strand of the tangle deforming
the edge of $\bF_{\mathrm{HL}}$ with $v_i$
to the end bounding the tangle strand deforming the edge with $v_j$.
Call a vector along the arc in this orientation $v$.
We define the sign of the arc relative to the face by
$$\sigma(F,a) := \mathrm{sgn}\det(v,v_i,v_j) = \mathrm{sgn}\det(-v,v_j,v_i)$$

\begin{center}
\begin{tikzpicture}[scale=1.3]
\draw[fill,gray,opacity=.5] (0,0)--(1.5,0)--(1.5,1)--(-.7,.7)--(0,0);
\draw[red, very thick] (0,0)--(-.7,.7);
\draw[green, very thick] (0,0)--(1.5,0);
\draw[red, very thick] (1.5,0)--(1.5,1);
\draw[black,thick, -stealth] (0,0)--(.3,0);
\draw[black,thick,-stealth] (0,0)--(-.2,.2);
\draw[black,thick,-stealth] (1.5,0)--(1.5,.3);
\draw[black,thick,-stealth] (1.5,0)--(1.2,0);
\draw[black] (-.07,.07)--(0.03,.07)--(.1,0);
\draw[black] (1.4,0)--(1.4,.1)--(1.5,.1);

\node at (.2,-.2) {$v$};
\node at (1.3,-.2) {$-v$};
\node at (.75,.5) {$F$};
\node at (.75,-.4) {$a$};
\node at (-.5,.2) {$v_i$};
\node at (1.8,.2) {$v_j$};
\end{tikzpicture}
\end{center}

Note that the opposite orientation on the arc leads
to $\mathrm{sgn} \det (-v,v_j,v_i),$ which is the same.
The definition therefore only depends on the orientation of $B$.
\end{definition}.

\begin{definition}
\label{def:facerelation}
Let $\bF'$ be a deformed foam with arc set $A$.
We define a relation $\sim$ on $\bZ^A$ by setting
$$\sum_{a\in \partial F} \sigma(F,a) \cdot a \sim 0,$$
for each \emph{internal} face $F$ of $\bF'$
\end{definition}

\begin{proposition}
Let $\bF$ be an ideal foam, and let $L$ be a smoothing
associated to a deformed foam $\bF'$ with arc set $A$.  Let
$\sim$ be as in Definition \ref{def:facerelation}.
Then $$H_1(L)\cong \bZ^A/\sim$$
\end{proposition}
\begin{proof}
We first need to prove that the map $a\mapsto \gamma_a$ respects the relation, i.e.
that $\sum_{a\in \partial F} \sigma(F,a) \cdot \gamma_a = 0$ in $H_1(L),$
for each internal face $F$.  Next we need to show that if there are $n$ arcs and $r$
internal faces, then the $r$ relations are independent.  Finally, the counting argument
of Lemma \ref{lem:nminusr} will show that the map from $\bZ^A/\sim$ to $H_1(L)$ is
surjective.

Let $\pi:L\to B$ be the covering map. 
Given an internal face $F$ of a foam with any orientation, let $F_T$ and $F_B$ be
the components of $\pi^{-1}(F)$, with their induced orientations. 
Consider $\widetilde{F}:=F_T-F_B$,
a two-chain on $L$.  Since $\pi$ is $1:1$ over the edges,
it follows that $\partial{\widetilde{F}} = \sum_{a\subset \partial F}\pm\gamma_a,$
where the sum is over the arcs of the boundary of $F$.
So it remains to prove that the choice of signs in Definition \ref{def:facerelation}, up to
an irrelevant overall sign.  \red{In the definition of $\sigma(F,a)$ if we give all the arcs
the induced orientation from the boundary of $F,$ we see that
the sign changes of $\sigma(F,a)$ agree with the sign changes....

To prove that the relations are independent, we note that....
a relation among the relations would require an internal region of the foam $\bF$, in contradiction
with our assumption that $\bF$ was an ideal foam.
}
\end{proof}



\subsubsection{The phase of a smoothing}

On general grounds, $L$ with $\partial L = S_\Gamma$ and
$b_1(L)=g = \frac{1}{2}b_1(S_\Gamma)$ defines a phase as the kernel of
the surjection $\pi:  H_1(S_\Gamma)\twoheadrightarrow H_1(L).$  Here we want to
understand this combinatorially when $L$ arises from a deformed foam $\bF'$,
in terms of its arcs and the edges of $\Gamma.$

Call a face $F$ of the foam $\bF'$ \emph{external} if it bounds an edge $e\in E_\Gamma$
of the cubic graph $\Gamma$.
Then similarly as in Definition \ref{def:facerelation}, we have for each external face
a relation in $H_1(L)$:
\begin{equation}
\label{eq:extfacerelation}
\pi(e) + \sum_{a\in \partial F} \mathrm{sgn}(F,a) \gamma_a = 0.
\end{equation}

\begin{proposition}
The relations of Equation \eqref{eq:extfacerelation} determine the map $\pi: H_1(S_\Gamma)
\to H_1(L),$ and therefore a phase.
\end{proposition}
\begin{proof}
To verify the relation, let $F$ be an external face endowed with an orientation and
consider the difference $\widetilde{F} := \widetilde{F}_{\mathrm{top}} - \widetilde{F}_{\mathrm{bot}}$ 
of the two lifts of $F$ to $L$, as a two-chain on $L$.
\red{We claim $\partial \widetilde{F} = e + \sum_{a\in \partial F}\sigma(F,a)\cdot \gamma_a.$}  
This proposition then follows immediately
since $H_1(S_\Gamma)\cong \bZ^{E_\Gamma}/\sim,$
as in Equation \eqref{eq:h1}\end{proof}

%Let ${\bf F}$ be a foam and let $s\in \cS$ be a smoothing.  Write
%$L$ for the corresponding Lagrangian and let
%${\bf F}_s$ be the associated deformed foam.  Write $A$ for the set of arcs of ${\bf F}_s$.
%We would like to construct a map $\bZ^A \to H_1(L)$ analogous to the construction
%from $\bZ^{E_\Gamma} \to H_1(S_\Gamma)$ for a cubic planar graph ---
%see Equation \eqref{eq:h1}.  To do so, we need to lift
%each arc consistently to an oriented loop of $L$.
%

\subsection{Face relations for foams}


\begin{proposition}
Let $\bF$ be an ideal foam filling a cubic graph $\Gamma$ with edge set $E$, and let $L$ be a smoothing
associated to a deformed foam $\bF'$ with arc set $A$, such that the corresponding tangle has no circle components.  Let
$\sim$ be as in Definition \ref{def:facerelation}.
Then $H_2(L)=0$, and we have an isomorphism 
$$
H_1(L)\cong \bZ^{A\cup E}/\sim
$$
such that the homology pushforward $H_1(\Lambda)\rightarrow H_1(L)$ is identified with the map induced by the inclusion $\bZ^{E}\hookrightarrow \bZ^{A\cup E}$. 
\end{proposition}
Since each generator associated to an edge $e\in E$ can be eliminated using the face relation for the corresponding external face of $\bF$, we obtain
\begin{corollary}
\label{cor:spanningarcs}
The group $H_1(L)$ is generated by the classes corresponding to arcs of the deformed foam, and we have an isomorphism 
$$
H_1(L)\cong \bZ^{A}/\sim.
$$
\end{corollary}
\begin{proof}
\red{Note added (EZ, 8/17/22):  need to correct for foams of non-simple graphs $\Gamma,$ e.g.~ones with bigons.  For example,
the necklace graph has no internal vertices but genus $g,$ since the external edges function as arcs.}
We prove the Proposition by induction on the number of internal vertices of the foam $\bF$, or equivalently on the number of tetrahedra in the dual tetrahedronation $\hat{\bF}$. The base case of a single tetrahedron is immediate from the explicit homotopies described in Section~\ref{sec:hlfoamdef}. We then have two cases to consider, depending on whether a tetrahedron is glued on by a single face, or instead by a pair of faces. To verify the induction step in the former case, let $\bF$ be a smoothed ideal foam, whose boundary is a cubic graph $\Gamma_{\bF}$ of genus $g$. The foam $\bF$ is dual to a tetrahedronation $\hat{\bF}$ of the 3-ball $B$. Recall that vertices of $\Gamma_{\bF}$, i.e. the boundary vertices of $\bF$, correspond to boundary faces of the tetrahedronation $\hat{\bF}$.

Now suppose $\Delta$ is a single tetrahedron together with a smoothed Harvey-Lawson foam $\bF_\Delta$ in it. Let us choose a vertex $v$ of $\Gamma_{\bF}$ along with a vertex $w$ of the cubic graph $\Gamma_\Delta$ on the boundary of the tetrahedron. Let us write $e_1,e_2,e_3$ for the three edges of $\Gamma_{\bF}$ incident to the vertex $v$ listed in cyclic order determined by the orientation, and similarly write  $\epsilon_1,\epsilon_2,\epsilon_3$ for the edges of $\Gamma_\Delta$ incident to $w$, but listed in opposite cyclic order. Each of these edges determines an external face of the corresponding foam, which we denote by $f_{e_i}$ or $f_{\epsilon_i}$. We glue the tetrahedron to $\hat{\bF}$ by identifying the tetrahedron face corresponding to $w$ with the boundary face of $\hat{\bF}$ corresponding to $v$ as indicated in Figure~\ref{fig:single-tetra-glue}, so that each edge $e_i$ is glued to the corresponding $\epsilon_i$ to form a new edge $\overline{e}_i$.  As a result of this gluing, we obtain a new ideal foam $\bF'$. 
%The corresponding cubic graph $\Gamma_{\bF'}$ on $\partial B$ is obtained from $\Gamma_\bF$ by blowing up the vertex $v$ as shown. 
\begin{center}
\begin{figure}[ht]

\begin{tikzpicture}

        \draw[fill=brown]  (-3,4.5) -- (-1, 1.5) -- (-5, 1.5) ;
        \draw[fill=brown]  (1,2)--(5,2)--(3,0.5);

		\node [] (0) at (-3, 4.5) {};
		\node [] (1) at (-1, 1.5) {};
		\node [] (2) at (-3, 4.5) {};
		\node [] (3) at (-5, 1.5) {};
		\node [label={\small $e_1$}] (4) at (-5, 3.5) {};
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt,label={$v$}] (5) at (-3, 2.5) {};
		\node [] (6) at (-3, 0.5) {};
		\node [label={\small $e_2$}] (40) at (-3, -0.15) {};
		\node [label={\small $e_3$}] (7) at (-1, 3.5) {};
		

		\node [] (8) at (3, 0.5) {};
		\node [] (9) at (1, 2) {};
		\node [] (10) at (5, 2) {};
		\node [] (11) at (3, 4.5) {};
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (12) at (2.25, 2.5) {}; %front-int-l
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (13) at (3.75, 2.5) {}; %front-int-r
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (14) at (2.75, 1.45) {}; %back-bottom
		\node [label={$w$}] (41) at (2.55, 0.85) {}; %back-bottom
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (15) at (3.25, 3.05) {}; %back-top
		\node [] (16) at (2, 3.25) {}; %left-edge-top
		\node [] (17) at (4, 3.25) {}; %right-edge-top
		\node [] (18) at (2, 1.25) {};%left-edge-bottom
		\node [] (19) at (4, 1.25) {}; %right-edge-bottom

        

		\node [] (20) at (9.475, 4.5) {};
		\node [] (21) at (10.725, 1) {};
		\node [] (22) at (9.475, 4.5) {};
		\node [] (23) at (6.725, 1.75) {};
		\node [] (24) at (8.975, 2.5) {};%{apex};
		\node [] (25) at (7.975, 2.75) {};
		\node [] (26) at (9.975, 2.75) {};
		\node [] (27) at (8.825, 1.25) {};
		\node [] (28) at (6.975, 3.25) {};
		\node [label=$\overline{e}_1$] (29) at (6.975, 3.25) {};%{left-ext};
		\node [label=$\overline{e}_3$] (30) at (10.975, 3.25) {};%{right-ext};
		\node [] (31) at (8.425, 0.5) {};%{bot-ext};
		\node [label=$\overline{e}_2$] (43) at (8.125, 0.25) {};
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (32) at (8.475, 2.75) {};%{l-int};
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (33) at (8.975, 2) {};%{b-int};
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (34) at (9.475, 2.75) {};%{r-int};








		\draw (0.center) to (1.center);
		\draw (2.center) to (3.center);
		\draw (3.center) to (1.center);
		\draw[blue] (4.center) to (5.center);
		\draw[blue] (5.center) to (7.center);
		\draw[blue] (5.center) to (6.center);
		\draw (9.center) to (8.center);
		\draw (8.center) to (10.center);
		\draw (11.center) to (9.center);
		\draw (11.center) to (10.center);
		\draw (9.center) to (10.center);
		\draw (11.center) to (8.center);
		\draw[blue] (12.center) to (16.center);
		\draw[blue,dashed] (16.center) to (15.center);
		\draw[blue,dashed] (15.center) to (17.center);
		\draw[blue,dashed] (15.center) to (14.center);
		\draw[blue] (12.center) to (13.center);
		\draw[blue] (17.center) to (13.center);
		\draw[blue,dashed] (14.center) to (18.center);
		\draw[blue,dashed] (14.center) to (19.center);
		\draw[blue] (12.center) to (18.center);
		\draw[blue] (13.center) to (19.center);
		
		\draw (20.center) to (21.center);
		\draw (22.center) to (23.center);
		\draw (23.center) to (21.center);
		\draw (22.center) to (24.center);
		\draw (24.center) to (23.center);
		\draw (24.center) to (21.center);
		\draw[blue] (29.center) to (25.center);
		\draw[blue] (30.center) to (26.center);
		\draw[blue] (27.center) to (31.center);
		\draw[blue] (25.center) to (32.center);
		\draw[blue] [in=135, out=45, looseness=1.25] (32.center) to (34.center);
		\draw[blue]	 [in=30, out=-90] (34.center) to (33.center);
		\draw[blue] [in=165, out=-90] (32.center) to (33.center);
		\draw[blue] (34.center) to (26.center);
		\draw[blue] (33.center) to (27.center);
\end{tikzpicture}

\caption{Gluing in a tetrahedron to $\hat{\bF}$ by a single face $\widehat{f}$, shaded in brown.}
\label{fig:single-tetra-glue}
\end{figure}
\end{center}

The set of faces of the new foam $\bF'$ may be described as follows. The internal faces of $\bF'$ are the same as those of $\bF$. The set of external faces of $\bF'$ consists of all those external faces of $\bF$ and $\bF_\Delta$ that correspond to edges of $\Gamma_{\bF}$ or $\Gamma_\Delta$ not incident to $v,w$, along with three faces $f_1,f_2,f_3$ obtained by gluing each $f_{e_i}$ to the corresponding $f_{\epsilon_i}$. 


We now turn our attention to the effect of this gluing at the level of the double covers of the ball. Let us write $\pi:L\rightarrow B, \pi_\epsilon:\mathrm{HL}_{\epsilon}\rightarrow B$ for the branched double covers corresponding to $\bF$ and $\bF_\Delta$ respectively, so that we have $L' = L \cup_{\pi^{-1}(\hat{f})} \mathrm{HL}_{\epsilon}$, where $\hat{f}$ is the face along which the tetrahedron $\Delta$ was glued to $\hat{\bF}$. This gluing is illustrated in Figure~\ref{fig:single-face-glue-cover}. 
\begin{center}
\begin{figure}[ht]

\begin{tikzpicture}[scale=.75]
	
		\node [] (0) at (-11.25, 1) {};
		\node [] (1) at (-3.25, 2) {};
		\node [] (2) at (-11.25, 9) {};
		\node [] (3) at (-3.25, 10) {};
		\node [] (4) at (-7.25, 1.5) {};
		\node [] (5) at (-7.25, 9.5) {};
		\node [] (6) at (-11.25, 5) {};
		\node [] (7) at (-3.25, 6) {};
		\node [] (8) at (-8, 4.5) {};%{h4l};
		\node [] (9) at (-6.75, 4){};% {h3l};
		\node [] (10) at (-6, 5) {};%{h2l};
		\node [] (11) at (-6.5, 6.5) {};%{h1l};
		\node [] (12) at (-7.75, 6.75) {};%{h0l};
		\node [] (13) at (-8.5, 5.75) {};%{h51};
		\node [] (14) at (0, 10) {};
		\node [] (15) at (8, 9) {};
		\node [] (16) at (0, 2) {};
		\node [] (17) at (8, 1) {};
		\node [] (18) at (4, 9.5) {};
		\node [] (19) at (4, 1.5) {};
		\node [] (20) at (0, 6) {};
		\node [] (21) at (8, 5) {};
		\node [] (22) at (3.25, 6.5) {};%{h1r};
		\node [] (23) at (4.5, 7) {};%{h0r};
		\node [] (24) at (5.25, 6) {};%{h5r};
		\node [] (25) at (4.75, 4.5) {};%{h4r};
		\node [] (26) at (3.5, 4.25) {};%{h3r};
		\node [] (27) at (2.75, 5.25) {};%{h2r};
		\node [] (28) at (-7.5, 7.75) {\tiny $e_3$};
		\node [] (29) at (-9.6, 7.25) {\tiny $e_1$};
		\node [] (32) at (8.25, 2.5) {};
		\node [] (34) at (4.25, 8) {\tiny $\epsilon_3'$};
		\node [] (35) at (6.75, 7.5) {\tiny $\epsilon_1'$};
		\node [] (36) at (2, 1.5) {};
		\node [] (37) at (-5, 6.10) {\tiny $e_2$};
		\node [] (40) at (1.5, 6.10) {\tiny $\epsilon_2'$};
		\node [] (41) at (-8.45, 7.75) {$-$};
		\node [] (42) at (-9.75, 6.25) {$+$};
		\node [] (43) at (-8.5, 3.75) {$-$};
		\node [] (44) at (-6, 3) {$+$};
		\node [] (45) at (-4.5, 4.5) {$-$};
		\node [] (46) at (-5.75, 7.25) {$+$};
		\node [] (47) at (2.5, 7.25) {$+$};
		\node [] (48) at (1.5, 4.5) {$-$};
		\node [] (49) at (2.75, 3.25) {$+$};
		\node [] (50) at (5.5, 3.75) {$-$};
		\node [] (51) at (6.75, 6.25) {$+$};
		\node [] (52) at (5.25, 8) {$-$};


		\draw[fill=brown]  (-8, 4.5) -- (-6.75, 4) -- (-6, 5)  -- (-6.5, 6.5)--(-7.75, 6.75) -- (-8.5, 5.75);
				\draw[fill=brown]  (3.25,6.5) -- (4.5,7) -- (5.25,6)  -- (4.75,4.5)--(3.5,4.25) -- (2.75,5.25);

		\draw[teal] (0.center) to (1.center);
		\draw[teal] (2.center) to (3.center);
		\draw[blue,<-] (4.center) to (5.center);
		\draw[magenta] (0.center) to (2.center);
		\draw[magenta] (1.center) to (3.center);
		\draw[red,->] (6.center) to (7.center);
		\draw[pink] (4.center) to (6.center);
		\draw[green,->] (1.center) to (2.center);
		\draw[pink] (7.center) to (5.center);
		\draw (8.center) to (9.center);
		\draw (9.center) to (10.center);
		\draw (10.center) to (11.center);
		\draw (11.center) to (12.center);
		\draw (13.center) to (12.center);
		\draw (8.center) to (13.center);
		\draw[teal] (14.center) to (15.center);
		\draw[teal] (16.center) to (17.center);
		\draw[blue,<-] (18.center) to (19.center);
		\draw[magenta] (14.center) to (16.center);
		\draw[magenta] (15.center) to (17.center);
		\draw[red,->] (20.center) to (21.center);
		\draw[pink] (18.center) to (20.center);
		\draw[green,->] (15.center) to (16.center);
		\draw[pink] (21.center) to (19.center);
		\draw (22.center) to (23.center);
		\draw (23.center) to (24.center);
		\draw (24.center) to (25.center);
		\draw (25.center) to (26.center);
		\draw (27.center) to (26.center);
		\draw (22.center) to (27.center);
\end{tikzpicture}


\caption{Gluing two copies of $\mathrm{HL}_{\epsilon}$ along the disk $\pi^{-1}(\hat{f})\subset \partial \mathrm{HL}_{\epsilon}\simeq T^2$. The set $\pi^{-1}(\hat{f})$ is shaded brown, and opposite pairs of boundary edges of the square are identified in the figure. The arrows on edges indicate the canonical lifts of the edges of the cubic graphs on $S^2$ to  cycles in $H_1(\Lambda)$. External faces of the foam are labelled by the corresponding sign of the primitive function.} 
\label{fig:single-face-glue-cover}
\end{figure}
\end{center}
%Recall that $\partial L = S_{\Gamma}$ is a closed surface of genus $g$, and that $\mathrm{HL}_{\epsilon}$ is a solid torus with boundary $\partial\mathrm{HL}_{\epsilon}\simeq T^2$. 
Now since the space $\pi^{-1}(\hat{f})$ is homeomorphic to a disk, the Mayer-Vietoris long exact sequence shows that $H_2(L')\simeq H_2(L)\oplus H_2({\mathrm{HL}_{\epsilon}})=0$. Similarly, it delivers an isomorphism
\begin{equation}
\label{mv-iso-1-face}
i_*+\iota_*: H_1(L)\oplus H_1({\mathrm{HL}_{\epsilon}}) \rightarrow H_1(L'),
\end{equation}
such that $[\overline{e}_i] = i_*([e_i])+\iota_*([\epsilon_i])$.
Hence all that remains is to verify the face relations for the faces $f_1,f_2,f_3$ of $\bF'$ obtained by gluing faces of $\bF$ to those of $\bF_\Delta$. But recall from \ref{def:arc-sign} that the definition of the sign of an arc $a$ relative to a face $f$ is entirely local,  depending only on the tangent vectors $v_i,v_j$ to the two edges of the deformed foam that meet $a$ and bound $f$. So if $a_0$ is the unique arc in the tetrahedron in $\hat{\bF}$ whose boundary contains the face $f$, and $a_1$ the corresponding arc in the tetrahedron $\Delta$, the sign of $a_0$ with respect to face $f_{e_i}$ in $\bF$ is identical to its sign with respect to face $f_i$ of the glued foam $\bF'$. Similarly, the sign of $a_1$ with respect to $f_{\epsilon_i}$ coincides with its sign with respect to $f_i$. The face relation for $f_i$ is therefore obtained as the sum of those for $f_{\epsilon_i}$ and $f_{e_i}$ under the isomorphism~\eqref{mv-iso-1-face}. 



We now consider the case of gluing in a tetrahedron by a pair of faces. Suppose that we fix an edge $e_0$ of $\Gamma_{\bF}$ connecting two vertices $v_1,v_2$, and correspondingly fix an edge $\epsilon_0$ of $\Gamma_{\Delta}$ connecting vertices $w_1,w_2$ of $\Delta$. Each vertex $v_i$ is dual to a boundary triangle of the tetrahedronation $\hat{\bF}$. Let us denote the edges of $\Gamma_{\bF}$ incident to $v_1$ by $e_0,e_1,e_2$, cyclically ordered in accordance with the orientation of $\partial B$, and  similarly write $e_0,e_3,e_4$ for the edges incident to $v_2$. We denote by $\epsilon_0,\epsilon_1,\epsilon_2$ the edges incident to $w_1$ but ordered with respect to the opposite of the orientation on $\Delta$, and similarly write $\epsilon_0,\epsilon_3,\epsilon_4$. We write $\epsilon_5$ for the remaining edge of $\Gamma_\Delta$ which is incident to neither $w_1$ nor $w_2$. We now glue the tetrahedron to the $\hat{\bF}$ by identifying the tetrahedron face corresponding to $w$ with the boundary face of $\hat{\bF}$ corresponding to $v$, so that each edge $e_i$ is glued to the corresponding $\epsilon_i$.  We denote by $\bF'$ the ideal foam produced as a result of this gluing.
\begin{center}
\begin{figure}[ht]
\begin{tikzpicture}
		\node [] (0) at (-6, 0) {};{rl};
		\node [] (1) at (0, 0) {};{rr};
		\node [] (2) at (-3.25, 2.75) {};{rt};
		\node [] (3) at (-2.5, -2.25) {};{rb};
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (4) at (-3.5, 1) {};%{Bt};
		\node [] (5) at (-4.75, 1.25) {};
		\node [] (6) at (-1.25, 1.25) {};
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (7) at (-4, 0.75) {};%{bl};
		\node [] (20) at (-3.85, 0.55) { $v$};;%{bl};
		\node [] (8) at (-0.75, -0.75) {};
		\node [] (10) at (-5.25, -0.5) {};
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (11) at (-3, -0.25) {};%{Bl};
		\node [] (12) at (-6.5, 2.5) {};{xt};
		\node [] (13) at (-6.5, -1.75) {};{xt};
		\node [] (14) at (0.5, 2.75) {};{xt};
		\node [] (15) at (0.75, -1.75) {};{xt};
		\node [circle,fill=blue,inner sep=0pt,minimum size=3pt] (16) at (-2, 0.75) {};%{br};
		\node [] (21) at (-2.1, 0.55) {$w$};%{br};

		\draw[red] (2.center) to (0.center);
		\draw[red] (0.center) to (3.center);
		\draw[red] (3.center) to (1.center);
		\draw[red] (2.center) to (1.center);
		\draw[red] (0.center) to (1.center);
		\draw[red,dashed] (2.center) to (3.center);
		\draw[blue] (12.center) to (5.center);
		\draw[blue] (13.center) to (10.center);
		\draw[blue] (14.center) to (6.center);
		\draw[blue] (8.center) to (15.center);
		\draw[blue] (5.center) to (4.center);
		\draw[blue] (4.center) to (11.center);
		\draw[blue] (10.center) to (11.center);
		\draw[blue] (11.center) to (8.center);
		\draw[blue] (4.center) to (6.center);
		\draw[blue,dashed] (5.center) to (7.center);
		\draw[blue,dashed] (10.center) to (7.center);
		\draw[blue,dashed] (7.center) to (16.center);
		\draw[blue,dashed] (6.center) to (16.center);
		\draw[blue,dashed] (16.center) to (8.center);
\end{tikzpicture}


\caption{The cubic graph (shown in blue)     produced by gluing a tetrahedron to $\hat{\bF}$ by a pair of faces is related to the orignal by a diagonal exchange.}
\label{fig:double-tetra-flip}
\end{figure}
\end{center}
\begin{center}
\begin{figure}[ht]

\begin{tikzpicture}

		\node [] (0) at (0.5, 1) {};
		\node [] (1) at (8.5, 2) {};
		\node [] (2) at (0.5, 9) {};
		\node [] (3) at (8.5, 10) {};
		\node [] (4) at (4.5, 1.5) {};
		\node [] (5) at (4.5, 9.5) {};
		\node [] (6) at (0.5, 5) {};
		\node [] (7) at (8.5, 6) {};
		\node [] (8) at (3.75, 4.5) {};%{h4l};
		\node [] (9) at (5, 4) {};%{h3l};
		\node [] (10) at (5.75, 5) {};%h2l};
		\node [] (11) at (5.25, 6.5) {};{h1l};
		\node [] (12) at (4, 6.75) {};{h0l};
		\node [] (13) at (3.25, 5.75) {};%{h51};
		\node [] (23) at (0.5, 6.5) {};%{md};
		\node [] (24) at (1.75, 2.5) {};%{MM};
		\node [] (25) at (6.75, 1.75) {};%{mdtR};
		\node [] (26) at (2.5, 1.25) {};%{mdtL};
		\node [] (29) at (7, 8.5) {};%{M};
		\node [] (30) at (7, 9.75) {};%{mdR};
		\node [] (31) at (8.5, 8.75) {};
		\node [] (32) at (2.5, 9.25) {};%{mdL};
		\node [] (33) at (0.5, 2.5) {};%{md};
		\node [] (34) at (8.5, 4.5) {};%{md};


		\draw[fill=brown]  (3.75, 4.5)-- (5, 4) --(5.75, 5)--(5.25, 6.5)--(4, 6.75)--(3.25, 5.75);
		\draw[fill=brown]  (4, 6.75)-- (2.5, 9.25) --(7, 9.75)--(7, 8.5)--(5.25, 6.5);
		\draw[fill=brown]  (3.75, 4.5)-- (1.75, 2.5) --(2.5, 1.25)--(6.75, 1.75)--(5, 4);

		\draw[blue,->>] (0.center) to (1.center);
		\draw[blue, ->>] (2.center) to (3.center);
		\draw[blue] (4.center) to (5.center);
		\draw[blue,->] (0.center) to (2.center);
		\draw[blue,->] (1.center) to (3.center);
		\draw[blue] (6.center) to (7.center);
		\draw[blue] (4.center) to (6.center);
		\draw[blue] (1.center) to (2.center);
		\draw[blue] (7.center) to (5.center);
		\draw[] (8.center) to (9.center);
		\draw[] (9.center) to (10.center);
		\draw (10.center) to (11.center);
		\draw (11.center) to (12.center);
		\draw (13.center) to (12.center);
		\draw (8.center) to (13.center);
		\draw (12.center) to (32.center);
		\draw (11.center) to (29.center);
		\draw (30.center) to (29.center);
		\draw (29.center) to (31.center);
		\draw (13.center) to (23.center);
		\draw (8.center) to (24.center);
		\draw (24.center) to (33.center);
		\draw (24.center) to (26.center);
		\draw (9.center) to (25.center);
		\draw (10.center) to (34.center);

\end{tikzpicture}
\caption{Shaded in brown is the subset $\pi^{-1}(\hat{\sigma})$ of $\partial \mathrm{HL}_{\epsilon} = T^2$. Edges of the cubic graph are shown in blue, and those of the dual triangulation in black. Since the opposite pairs of blue boundary edges are identified, the space $\pi^{-1}(\hat{\sigma})$ is homeomorphic to a cylinder.}
\label{fig:cylinder-glue}
\end{figure}
\end{center}

%The corresponding cubic graph $\Gamma_{\bF'}$ on $\partial B$ is obtained from $\Gamma_{\bF}$ as shown in Figure~\eqref{}. 
In contrast to the case of gluing by a single triangle, note that the cubic graphs $\Gamma_{\bF'}$ and $\Gamma_{\bF}$ have the same genus: indeed, the two are related by a single diagonal exchange/edge mutation, as illustrated in Figure~\ref{fig:double-tetra-flip}. Under the correspondence between edges of the cubic graph and external faces of the foam, the set of external faces of $\bF'$ is thus in natural bijection with that of $\bF'$: the latter contains of all four external faces $\{f_i, i=1,\ldots 4\}$ obtained by gluing each face $f_{e_i}$ to the corresponding $f_{\epsilon_i}$, along with the external face coming from $f_{\epsilon_5}$.  On the other hand, we now have a new \emph{internal} face $f_0$ created by gluing $f_{e_0}$ to $f_{\epsilon_0}$. By assumption, the smoothing of the foam in $\Delta$ is chosen such that the tangle in the glued foam $\bF'$ has no circle components; this is equivalent to requiring that at least one of the faces $f_{e_0},f_{\epsilon_0}$ contains an arc as part of its boundary. 

We now consider the gluing of double covers $\pi:L\rightarrow B, \pi_\epsilon:\mathrm{HL}_{\epsilon}\rightarrow B$. Once again we have $L' = L \cup_{\pi^{-1}(\hat{\sigma})} \mathrm{HL}_{\epsilon}$, where $\hat{\sigma}$ is the quadrilateral along which the tetrahedron $\Delta$ is glued to $B$. As shown in Figure~\ref{fig:cylinder-glue} the space $\pi^{-1}(\hat{\sigma})$ is homeomorphic to a cylinder $C$. We fix the isomorphism $H_1(C)\simeq \mathbb{Z}\{\gamma\}$, where we take the generator $\gamma$ to be the oriented loop on $\partial \mathrm{HL}_\epsilon$ given by canonical lift of the edge $\epsilon_0$ of $\Gamma_{\Delta}$.  The relevant part of Mayer-Vietoris sequence then reads
\begin{equation}
\label{mv-iso-2-face}
0\rightarrow H_2(L')\rightarrow \mathbb{Z}\{\gamma\}\rightarrow H_1(L)\oplus H_1({\mathrm{HL}_{\epsilon}}) \rightarrow H_1(L')\rightarrow 0.
\end{equation}
By our assumption that at least one of the faces $f_{e_0},f_{\epsilon_0}$ contains an arc as part of its boundary, we see that the map 
$$
i_*\oplus (-\iota_*) : \mathbb{Z}\{\gamma\}\rightarrow H_1(L)\oplus H_1({\mathrm{HL}_{\epsilon}})
$$ is injective. Hence $H_2(L')=0$, and 
$$
H_1(L') \simeq \frac{H_1(L)\oplus H_1({\mathrm{HL}_{\epsilon}})}{\mathbb{Z}\{\gamma\}}.
$$
The face relations for all external faces of $\bF'$ now follow from this description of $H_1(L')$ exactly as in the case of the single-triangle gluing. Finally, since 
$$
\left(i_*\oplus (-\iota)_*\right)(\gamma)  = ([e_0],[\epsilon_0]),  
$$
we see from the isomorphism~\eqref{mv-iso-2-face} that the relation in $H_1(L')$ corresponding to the new internal face $f_0$ is also obtained as the sum of the relation corresponding to $f_{e_0}$ in $H_1(L)$ with that corresponding to $f_{\epsilon_0}$ in $H_1({\mathrm{HL}_{\epsilon}})$. This completes the proof of the Lemma.





\end{proof}


\subsection{Example -- triangular prism}
\label{sec:prism}

Let $\Gamma$ be the edge graph of a triangular prism and let $\bF'$
be the deformed foam pictured here:

\begin{center}
\begin{tikzpicture}[scale=1.3]
\pgfmathsetmacro{\Ax}{0}
 \pgfmathsetmacro{\Ay}{3}
 \pgfmathsetmacro{\Bx}{2.3}
 \pgfmathsetmacro{\By}{3.3}
 \pgfmathsetmacro{\Cx}{1}
 \pgfmathsetmacro{\Cy}{4}
 \pgfmathsetmacro{\Dx}{0}
 \pgfmathsetmacro{\Dy}{0}
 \pgfmathsetmacro{\Ex}{2.3}
 \pgfmathsetmacro{\Ey}{0.3} 
\pgfmathsetmacro{\Fx}{1}
 \pgfmathsetmacro{\Fy}{1}
 \coordinate (A) at (\Ax,\Ay);
 \coordinate (B) at (\Bx,\By);
 \coordinate (C) at (\Cx,\Cy);
 \coordinate (D) at (\Dx,\Dy);
 \coordinate (E) at (\Ex,\Ey);
  \coordinate (F) at (\Fx,\Fy);
 \coordinate (Amid) at (.7,1.5);
  \coordinate (Amidtext) at (.7-.3,1.5);
 \coordinate (Amid2) at (.5,1.7);
 \coordinate (Bmid) at (1.5,1.6);
 \coordinate (Bmid2) at (1.7,1.7);
  \coordinate (Bmidtext) at (1.6,1.5);
 \coordinate (Cmid) at (1.32,2.3);
 \coordinate (Cmid2) at (1.2,2.1);
  \coordinate (Cmidtext) at (1.15,2.25);

 \coordinate (ACmid) at (\Ax/2+\Cx/2-.4,\Ay/2+\Cy/2);
 \coordinate (BCmid) at (\Bx/2+\Cx/2+.3,\By/2+\Cy/2+.1);
 \coordinate (ABmid) at (\Ax/2+\Bx/2+.4,\Ay/2+\By/2-.3);
 \coordinate (DFmid) at (\Dx/2+\Fx/2+.2,\Dy/2+\Fy/2-.1);
 \coordinate (EFmid) at (\Ex/2+\Fx/2,\Ey/2+\Fy/2+.2);
 \coordinate (DEmid) at (\Dx/2+\Ex/2+.2,\Dy/2+\Ey/2-.25);
 \coordinate (ADmid) at (\Ax/2+\Dx/2-.3,\Ay/2+\Dy/2);
 \coordinate (CFmid) at (\Fx/2+\Cx/2-.3,\Fy/2+\Cy/2+.1);
 \coordinate (BEmid) at (\Bx/2+\Ex/2+.3,\By/2+\Ey/2);
 

\draw[fill,black,opacity=.4] (Amid2)--(Amid)--(Bmid)--(Bmid2)--(Cmid2)--(Amid2);
\draw[fill,red,opacity=.4] (A)--(Amid2)--(Cmid2)--(Cmid)--(C)--(A);

\draw[red, thick] (D)--(Amid)--(Bmid)--(B);
\draw[red, thick] (A)--(Amid2)--(Cmid2)--(Bmid2)--(E);
\draw[red, thick] (C)--(Cmid);
\draw[red, thick, dashed] (Cmid)--(F);
\draw[green, ultra thick] (Amid)--(Amid2);
\draw[green, ultra thick] (Cmid)--(Cmid2);
\draw[green, ultra thick] (Bmid)--(Bmid2);

\draw[blue,thick] (A)--(B)--(C)--(A)--(D)--(E)--(B); 
\draw[blue,thick,dashed] (D)--(F)--(E);
\draw[blue,thick,dashed] (F)--(C);

\node at (Amidtext) {$b$};
\node at (Bmidtext) {$c$};
\node at (Cmidtext) {$a$};

\node at (ACmid) {$T_1$};
\node at (BCmid) {$T_2$};
\node at (ABmid) {$T_3$};
\node at (DFmid) {$B_1$};
\node at (EFmid) {$B_2$};
\node at (DEmid) {$B_3$};
\node at (ADmid) {$L_1$};
\node at (CFmid) {$L_2$};
\node at (BEmid) {$L_3$};


\end{tikzpicture}
\end{center}

Write $G$ for the gray face and $P$ for the pink face.  Then $\sigma(P,a) = 1,$
and from Equation \eqref{eq:extfacerelation}, $P$ gives the relation $$\pi(T_1)+\gamma_a = 0.$$  
In total, the external face relations give
$$\begin{array}{rclccrclccrcl}
\pi(T_1)+\gamma_a &=& 0 && \pi(L_1)+\gamma_b &=& 0&& \pi(B_1)-\gamma_b - \gamma_a &=& 0\\
\pi(T_2)-\gamma_a-\gamma_c &=& 0 && \pi(L_2)&=&0&& \pi(B_2)+ \gamma_a &=& 0\\
\pi(T_3)-\gamma_b &=& 0&&\pi(L_3)+\gamma_c &=& 0&& \pi(B_3)- \gamma_c &=& 0
\end{array}$$
We also have the internal (gray) face relation, and since $\sigma(G,b)=\sigma(G,c)=1,$ we see
$$\gamma_b+\gamma_c = 0.$$
The relations are consistent with the face relations from $\Gamma$.  For example, the sum
$T_1 + T_2 + T_3 = 0$, and this implies $\pi(T_1+T_2+T_3)=0,$ or
$\gamma_b + \gamma_c = 0,$ and this is true by the internal face relation.
The other face relations are consistent, as well. 

So $\pi$ indeed descends from a map from $\bZ^A$ to
one from $H_1(S_\Gamma)\cong \bZ^{E_\Gamma}/\sim,$ giving a map to $H_1(L)=\bZ^A/\sim$.
$H_1(S_\Gamma)$ is rank-$4$ and we can take Darboux generators $T_1,T_2;B_2,B_1$
(careful about the cyclic order on the back side of the prism:  $\overline{\omega}(B_2,B_1)=1$).
$H_1(L)$ is rank-$2$ and we can take generators $\gamma_a,\gamma_b$.
With these generators,
$$\pi(T_1) = -\gamma_a, \quad
 \quad \pi(T_2) = \gamma_a - \gamma_b,\quad
 \pi(B_2) = -\gamma_a,\quad
 \pi(B_1) = \gamma_a+\gamma_b
.$$
We can see that the kernel of $\pi$ is generated by
$\mu_1 := -(T_1+T_2+B_1+B_2)$ and
$\mu_2 := T_1 - B_2,$
and is indeed isotropic.
A framing $H_1(L)\hookrightarrow H_1(S_\Gamma)$
must send $\gamma_a$ to $-T_1 + \alpha \mu_1 + \beta \mu_2$
and $\gamma_b$ to $B_1 + B_2 + \gamma \mu_1 + \delta \mu_2$
The image is isotropic if $\beta =\gamma,$ so the different framings
for this phrase are parametrized
by symmetric $2\times 2$ integer matrices $\binom{\tiny{\alpha\;\beta}}{\tiny{\beta\;\delta}}.$





\subsection{Open Gromov-Witten Conjectures}

Consider a cluster chart $\cP_\Gamma$ of $\cP$ defined by a Lagrangian $L$
with $\partial L = S_\Gamma.$
Given a splitting (phase and framing), a basis $e_i$ for $H_1(L)$ determines a Darboux-conjugate
dual basis $e_i'$ (with $\omega(e_i,e_j') = \delta_{i,j})$
and corresponding torus coordinates $(x_i,y_j)$.
The splitting $A$ thus identifies
$\cP_\Gamma \cong T^*H^1(L;\bC^*)/H_1(L;\bZ).$
The moduli space $\cM\subset T^*H^1(L;\bC^*)$ lifts to $\widetilde{\cM}_\Gamma
\subset T^*H^*(L;\bC^*)$, and we call a primitive function $W_\Gamma^{(A)}$
so that $\widetilde{\cM}_\Gamma \cong \mathrm{Graph}(dW_\Gamma^{(A)})$ a
\emph{superpotential}.

Generalizing the constructions of Ooguri-Vafa \cite{OV},
Aganagic-Vafa \cite{AV},
and Aganagic-Klemm-Vafa \cite{AKV},
and incorporating the integrality conditions of \cite{OV},
we make the following conjecture.
\begin{conjecture} \label{conj:disks}
The superpotential $W_\Gamma^{(A)}$ is the generating function for
holomorphic disk invariants of $L$ in framing $A$.  It has an expansion
as $$W_\Gamma^{(A)}(x_1,...,x_g) = \sum_{d \in \bZ_{\geq 0}^g \setminus \{0\}}
n_{d}^{(A)} \mathrm{Li}_2(x^d),$$
where $x^d = x_1^{d_1}\cdots x_g^{d_g},$
$\mathrm{Li}_2(x) = \sum_{n\geq 0}x^n/n^2,$
 and the $n^{(A)}_d$ are integers, the Ooguri-Vafa disk invariants
 in phase and framing $A$.
\end{conjecture}

\begin{remark}
The conjecture is a bit premature, as the
construction of open Gromov-Witten invariants is still a work in progress,
though we are told
that a proper definition of these enumerative invariants
should incorporate the splitting $A$.\footnote{We thank Jake Solomon
and Sara Tukachinsky for explaining this to us.}
\end{remark}

The quantization of the above leads to
higher-genus open-Gromov-Witten conjectures, as follows.

The cluster variety $\cP$ has a quantization, which in each symplectic chart
$(\cP_\Gamma,\omega)$ can identified with 
the quantum torus algebra $\cT^q$ by 
$X_e X_{e'} = q^{\omega(e,e')}X_{e'}X_e$ for $e,e' \in H_1(S_\Gamma)$.
This is equivalent to $X_e X_{e'} = q^{\frac{1}{2}\omega(e,e')}X_{e+e'}.$
\footnote{Notation $\cT := H^1(S_\Gamma;\bC^*).$  An element $e\in H_1(S_\Gamma)$ defines a coordinate function $X_e$ on $\cT$ by $X_e(\lambda) = \lambda(e).$
If $e\in \mathrm{Ker}(\pi:H_1(S_\Gamma)\to H_1(L)),$
then $X_e$ makes sense as a coordinate on $H_1(L;\bC^*)$....}
%Given a splitting, any basis $e_i$ for $H_1(L)$ determines a Darboux-conjugate
%dual basis $e_i'$ (with $\omega(e_i,e_j') = \delta_{i,j})$
%and corresponding torus coordinates $(x_i,y_j)$.
%whose value on $\lambda
%\in H^1(S_\Gamma,\bC^*)$ is defined by $x_i(\lambda) = \lambda(e_i)$
%and $y_j(\lambda) = \lambda(e_j')$. 
Given our splitting $A$ and basis $e_i$ for $H_1(L),$ the 
generators $x_i,y_j$ 
obey $y_i x_i = q x_i y_i,$ with
all other pairs commuting.  This identifies $\cT^q$ with
$\cD:=\bQ(q)[x_i^{\pm},y_i^\pm].$

The quantization of $\cM_\Gamma \subset \cP_\Gamma \cong T^*(\bC^*)$
is a left ideal $\cI\subset \cD$, and we have defined generators $L_i \in \cD$,
one for each face of $\Gamma.$
Recall the regular $\cD$-module defined by $\bQ[t_1,...,t_n],$ with action of $x_i$ and $y_j$ on
an element $f$ defined as follows:  $(x_i \cdot f)(t_1,...,t_n) = t_if(t_1,...,t_n)$
and $(y_j \cdot f)(t_1,...,t_n) = f(t_1,...,qt_j,...,t_n).$  (This is just the exponentiated
action of position and momentum operators, with $q = e^\hbar$.)
We define the (algebraic) \emph{wavefunction} $\Psi_\Gamma^{(A)}$ to be a cyclic vector
generating the $\cD$-module $\cD/\cI D,$ one obeying $L_i\Psi_\Gamma = 0$ for all $i$.

In the spirit of \cite{OV} and \cite{AENV}, which investigated wavefunctions in the context of knot conormals in large-$N$ duality, we make the following conjecture.

\begin{conjecture}
The wavefunction $\Psi_\Gamma^{(A)}$ is the generating function for
all-genus open Gromov-Witten invariants of $L$ in framing $A$.  It has an expansion
as $$\Psi_\Gamma^{(A)}(x_1,...,x_g) = \prod_{s\geq 0}
\prod_{d \in \bZ_{\geq 0}^g \setminus \{0\}}
\Phi(x^dq^s)^{n_{d,s}^{(A)} },$$
where $x^d = x_1^{d_1}\cdots x_g^{d_g},$
$\Phi(x) = \prod_{n\geq 0}\frac{1}{1-q^nx}$
 and the $n^{(A)}_{d,s}$ are integers, the higher-genus Ooguri-Vafa invariants
 in phase and framing $A$.
\end{conjecture}



